Benchmarking VLMs' Reasoning About Persuasive Atypical Images

Vision language models (VLMs) have shown strong zero-shot generalization across various tasks, especially when integrated with large language models (LLMs). However, their ability to comprehend rhetorical and persuasive visual media, such as advertisements, remains understudied. Ads often employ atypical imagery, using surprising object juxtapositions to convey shared properties. For example, Fig. 1 (e) shows a beer with a feather-like texture. This requires advanced reasoning to deduce that this atypical representation signifies the beer's lightness. We introduce three novel tasks, Multi-label Atypicality Classification, Atypicality Statement Retrieval, and Aypical Object Recognition, to benchmark VLMs' understanding of atypicality in persuasive images. We evaluate how well VLMs use atypicality to infer an ad's message and test their reasoning abilities by employing semantically challenging negatives. Finally, we pioneer atypicality-aware verbalization by extracting comprehensive image descriptions sensitive to atypical elements. Our findings reveal that: (1) VLMs lack advanced reasoning capabilities compared to LLMs; (2) simple, effective strategies can extract atypicality-aware information, leading to comprehensive image verbalization; (3) atypicality aids persuasive advertisement understanding. Code and data will be made available.

==> dumps/method.tex <==
\section{Approach}



% % % 
% % % % %  Atyplicality Statement Retrieval
% % % 
\textbf{Atyplicality Statement Retrieval.}


As observed in Fig. \ref{fig:sub5} knowing the atypicality relation between the objects in the image can improve the performance of the model in action-reason detection task. So, to find the atypicality relation in the image, we introduce the task of atypicality statement retrieval, to be utilized in action-reason detection and image understanding task. 



MAC is a very challenging task as it requires the model to comprehend the atypicality definition and detect the atypicality in the image accordingly. Moreover, the detected merely atypicality label directly is not very useful for action-reason detection task. On the other hand, these four atypicality categories can be also written in a form of  atypicality statements $\mathcal{S}_{\mathcal{A}}$ describing the relation between two objects\footnote{the ground-truth atypical objects are provided by PittAd data.} (aka 'primary object' and 'secondary object'). 
% The 'primary object' is the main object in the image, while the 'secondary object' is utilized to convey a message, such as an attribute associated with the 'secondary object' to the user. This allows us to define an atypicality statement for each atypicality:


 ASR involves a model choosing the most accurate description of the atypical relation between the objects in the image, distinguishing correct from incorrect options.
To construct the correct and incorrect options, we initially formulate a statement for each category of atypicality:


After retrieving the correct primary concept (object1),  secondary concept (object2) and the correct category of the atypicality from the annotations in original dataset \cite{hussain2017automatic} and using the the definition of statements, generated the correct statements. To create incorrect options, we employ three strategies: replacing the objects with those from another image, altering the atypicality relationship while keeping the original objects, and swapping the primary and secondary objects to form a misleading statement. This process ensures a comprehensive test of a model's ability to understand and interpret atypical visual relationships.





% A-R netagive genration

To make the action-reason task more challenging, we modified the options in the original \cite{hussain2017automatic} dataset, keeping the correct options and replacing the incorrect options with semantically different options. Previously, incorrect options were easily distinguishable, being visually unrelated to the correct answer as they were chosen from the correct options in other images. To generate new incorrect options,  we utilized the GPT-4 API to generate alternatives that are lexically similar to the correct choice but differ significantly in meaning through changes in one of the following forms:
\begin{itemize}
    \item \textbf{Action}:  Modify the action while keeping the reason unchanged. For example, \textit{I should buy Heineken beer, because it is refreshing}, becomes \textit{I shouldn't buy Heineken Beer, because it is refreshing}.
    \item \textbf{Reason}: Keep the action the same but change the reason. For example: \textit{I should buy Heineken beer, because it is refreshing} becomes \textit{I should buy Heineken beer, because it is not refreshing.}
    \item \textbf{Adjective}: Change or add an adjective to change the meaning of the sentence while keeping the rest of the sentence unchanged. For example, \textit{I should buy Heineken beer, because it is refreshing} becomes, \textit{I should buy Heineken beer, because it is tasty}.
    \item \textbf{Object}: Change or add an object to change the message. For example, \textit{I should buy Heineken beer, because it is refreshing} becomes, \textit{I should buy Corona beer, because it is refreshing}
    \item \textbf{Semantic}: With minimum change in the sentence, change the semantic of the sentence. For example, \textit{I should buy Heineken beer, because it is refreshing}, becomes \textit{I should buy Heineken vodka, because it is strong}.
\end{itemize}





% final approach



% While the former aims to provide a clear description of the scene and objects, the latter aims to describe the unusual aspect of the image, which is more aligned with the concept of atypicality. However, as illustrated in Table~\ref{table:res}, we observe that while both prompts are useful compared to the VLM baselines and object/text-only baseline, they provide different and complementary information. Hence, we propose using an LLM (i.e., GPT-4) to combine all information obtained with previous prompts (i.e., $V$, $T$, $IN$, and $UH$) and produce a clear verbalization $\mathcal{T}_{\mathcal{V}}$.















% after getting the description of the image in the first step and the most accurate atypicality statement to describe the relation between the objects in the second step, we combine them as the context for an LLM and prompt the LLM to find the most accurate interpretation for the advertisement image.


% Action-reason retrieval is the task of finding the most accurate interpretation for the advertisement image among the input options. Each option is a statement consisting of the action that the image convinces the audience to take and the reason why the audience should take the action. In this work unlike the original dataset we make the incorrect options semantically different from correct options to make the task more challenging for vision models.




%To better understand the hidden message in advertisement images we propose a framework by combining the descriptive capability of VLMs and reasoning capability of LLMs. This approach starts with utilizing VLMs to generate a detailed analysis of the input image, including detailed description generation, text recognition, and identifying up to five objects. Using the identified object list and the atypicality relations outlined in section \ref{sec:atyp-understanding}, a list of potential atypicality statements was crafted, including both correct and incorrect statements. Next, we employ an LLM to given the description of the image, recognized texts and list of potential atypicality statements, detect the best statement to describe the atypicality relation between the objects in the image. This chosen statement, along with the image description and recognized text, forms the prompt for an LLM to accurately identifying the best action-reason statement for interpreting the image. Fig. \ref{fig:model} shows this framework.



% Following prior works \cite{hussain2017automatic,ye2021breaking}, we focus on the Ad understanding task (i.e., action-reason retrieval) in order to evaluate the impact of atypicality on understanding the visual media. \cite{hussain2017automatic} provided three action-reason statements for each image. These action-reason statements may have different plausible reasons for the same action, e.g. \textbf{Todo: Provide example}. Therefore, given three plausible (i.e., positive) and many implausible (i.e., negative) action-reason statements, the task is to detect all plausible action-reason statements. 








==> figures/ASR_error_analysis.tex <==
\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.25\textwidth]{images/results/ASR_error_analysis.png}
    \caption{Error analysis of ASR task on full-set. Distribution of incorrect options chosen by different models over different types of ASR negative options.}
    \label{fig:ASR_Error_Analysis}
\end{figure}


==> figures/error_distribution_analysis.tex <==



% \begin{figure}[ht]
% \centering

% \begin{subfigure}[b]{0.3\textwidth}
%     \includegraphics[width=\textwidth]{images/results/ASR_error_analysis.png}
%     \caption{Error analysis of ASR task on full-set. Distribution of incorrect options chosen by different models over different types of negatives.}
%     \label{fig:ASR_GPT4_LLAVA_ERR_ANALYSE}
% \end{subfigure}
% \hfill
% \begin{subfigure}[b]{0.6\textwidth}
%     \includegraphics[width=\textwidth]{images/results/error_analysis_barchart.png}
%     \caption{Error analysis of ARR task on full-set. Distribution of incorrect options chosen by different models over different types of hard negatives.}
%     \label{fig:ARR_ERR_ANALYSE}
% \end{subfigure}
% \hfill
% % \begin{subfigure}[b]{0.3\textwidth}
% %     \includegraphics[width=\textwidth]{images/results/error_analysis_gpt4.png}
% %     \caption{Discriminative Model}
% %     \label{fig:sub3}
% % \end{subfigure}

% \caption{Error analysis of ARR task on full-set}
% \label{fig:test}

% \end{figure}


\begin{figure}[!tp]
    \centering
    \includegraphics[width=0.5\textwidth]{images/results/ASR_Analyse.png}
    \caption{Error analysis of ARR task on full-set. Distribution of incorrect options chosen by different models over different types of hard negatives.}
    \label{fig:ARR_Error_Analysis}
\end{figure}



==> figures/intro_example_table.tex <==
% \begin{tabular}{c@{\hspace{0.pt}}c@{\hspace{0.pt}}c|c@{\hspace{0.pt}}}
% % First Column (Figure 1a)
% \multirow{2}{*}[1.in]{ % Adjust the value in [] to align the images vertically
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth,height=2.5in]{images/intro/example1.png} % Adjust height as needed
%   \caption{First subfigure}
%   \label{fig:sub1}
% \end{subfigure}
% }
% &
% % Second Column (Figure 1b)
% \multirow{2}{*}[1.in]{ % Adjust the value in [] to align the images vertically
% \begin{subfigure}{.15\textwidth}
%   \centering
%   \includegraphics[width=\linewidth,height=2.5in]{images/intro/example2.jpg} % Adjust height as needed
%   \caption{Second subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% }
% &
% % Third Column, First Row (Figure 1c)
% \begin{subfigure}{.19\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/intro/example3.jpg} % Replace with your image
%   \caption{Third subfigure}
%   \label{fig:sub3}
% \end{subfigure}
% \\
% &
% &
% % Third Column, Second Row (Figure 1d)
% \begin{subfigure}{.20\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/intro/example4.png} % Replace with your image
%   \caption{Fourth subfigure}
%   \label{fig:sub4}
% \end{subfigure}
% &
% % The fourth column is already set to span both rows (Figure 2)
% \end{tabular}
% \caption{A composite image with subfigures.}

==> figures/intro_examples_plot.tex <==
% \newcommand{\rulesep}{\unskip\ \vrule\ }


\begin{figure*}[!tp]
\centering
% Left side: 4 examples in 2 rows, with its own caption
\begin{minipage}[t]{0.6\textwidth}
    % Row 1
    % \vspace{-150pt}
    \begin{subfigure}[t]{0.9\linewidth}
        \includegraphics[width=\linewidth]{images/intro/intro_all.png}
        % \caption{}
        % \label{fig:intro_a}
    \end{subfigure}
    \caption{\textbf{Atypicality categories.} We study 4 types of atypicality from the taxonomy in \cite{yeinterpreting}:  Texture Replacement 1, Texture Replacement 2,  Object Inside Objects, Object Replacement (defined in Sec.~\ref{sec:method}).} % Caption for the left side
    \label{fig:intro_examples}
\end{minipage}
\hfill
% \rulesep
% Right side: Histogram plot, with its own caption
\begin{minipage}[t]{0.35\textwidth}
    \vspace{-100pt} % Align the top of the minipage with 
% \centering
\includegraphics[width=1\linewidth]{images/intro/intro_plot_2.png}
    % \vspace{10pt}
    \caption{We %sampled 250 images from the dataset and 
    input the GT atypicality statement (Sec.~\ref{sec:atyp-tasks}) along with the image and asked the model to retrieve one correct action-reason statement. Atypicality greatly improves reasoning.}
    \label{plot:intro_motivation}
\end{minipage}
\end{figure*}



% \begin{figure}[ht]
% \centering
% \begin{tabular}{ccc}
% % First Column
% \multirow{2}{*}{ % Adjust the value in [] to align the images vertically
% \begin{subfigure}{.2\textwidth}
%   \centering
%   \includegraphics[width=\linewidth,height=3in]{images/intro/intro1.jpg} % Replace with your image
%   \caption{First subfigure}
%   \label{fig:sub1}
% \end{subfigure}
% }
% &
% % Second Column
% \multirow{2}{*}{ % Adjust the value in [] to align the images vertically
% \begin{subfigure}{.2\textwidth}
%   \centering
%   \includegraphics[width=\linewidth,height=3in]{images/intro/intro2.png} % Replace with your image
%   \caption{Second subfigure}
%   \label{fig:sub2}
% \end{subfigure}
% }
% &
% % Third Column, First Row
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/intro/intro3.jpg} % Replace with your image
%   \caption{Third subfigure}
%   \label{fig:sub3}
% \end{subfigure}
% \\
% &
% &
% % Third Column, Second Row
% \begin{subfigure}{.3\textwidth}
%   \centering
%   \includegraphics[width=\linewidth]{images/intro/intro3.jpg} % Replace with your image
%   \caption{Fourth subfigure}
%   \label{fig:sub4}
% \end{subfigure}
% \end{tabular}
% \caption{A composite image with subfigures.}
% \label{fig:test}
% \end{figure}



==> figures/intro_motivation_plot.tex <==
\begin{figure}[!tp]
\centering
\includegraphics[width=0.7\linewidth]{images/intro/intro_plot_2.png}
    % \vspace{10pt}
    \caption{We %sampled 250 images from the dataset and 
    input the GT atypicality statement (Sec.~\ref{sec:atyp-tasks}) along with the image and asked the model to retrieve one correct action-reason statement. Atypicality greatly improves reasoning.}
\end{figure}

==> figures/llava_example.tex <==
\begin{figure*}[!tp]
    \centering
    \includegraphics[width=1\textwidth]{images/method/example.png}
    \caption{\textbf{An example of output of LLAVA on describing the image and reasoning on the images. I indicates the input input image, IN and UH are the the IN and UH descriptions generated by LLAVA. Incorrect/correct phrases/statements are given and are highlighted in \textcolor{red}{red}/\textcolor{green}{green}. The selected options by LLAVA are bold.}}
    \label{fig:LLAVA_example}
\end{figure*}

==> prompts/combine_prompt_Vicuna.tex <==
\begin{lstlisting}[caption={\textbf{Prompt format for combining verbalizations to generate $\mathcal{T}_\mathcal{V}$ based on Vicuna}. \textcolor{highlight-blue}{Blue} denotes elements added dynamically.},label={list:prompt_combine_vicuna}]
A chat between a curious human and an artificial intelligence assistant. The assistant gives helpful, detailed, and polite answers to the human's questions about an image. Analyze each assistant's response carefully, then combine the information, and summarize the combined information in a way that is useful for further question/answering tasks. Your answer must be a high-quality summary of the information.

(*@\textbf{Input Question-Anwers:}@*)

Question: 
    What are the non-textual objects visible in this image? Carefully output AT MOST top 5 objects. If there are more than 5 objects, output major/important objects according to the image. Words/Texts do not consider as objects. Separate with comma
Answer:
      (*@\textcolor{highlight-blue}{$V$ (List of top-5 objects)}@*)
Question:
    You are an OCR expert. What are the text messages in the image?
Answer:
    (*@\textcolor{highlight-blue}{$T$ (List of scene-tests)}@*)
Question:
    Describe the image in detail.
Answer:
    (*@\textcolor{highlight-blue}{$IN$ (Image Description)}@*)
Question:
    What is unusual about this image?
Answer:
    (*@\textcolor{highlight-blue}{$UH$ (Image Unusualness)}@*)
Carefully combine the above information given by the assistant.\end{lstlisting}


==> sections/ECCV_dumps/abstract_ECCV.tex <==
\begin{abstract}
Computational understanding of the strategies that visual persuasive media employ is important for deciphering the messages they aim to convey. In this paper, we focus on one particular strategy, which is the creation of atypical imagery in advertising, where the surprising juxtaposition of objects conveys they share a property. Atypical imagery is very creative and thus challenging for classic vision algorithms to capture, but recent vision-language foundational models (VLMs) show some promise. However, more complex reasoning capabilities are needed to connect the atypical strategies to the broader message the ad aims to convey. We thus utilize these VLMs to provide a verbalization of the atypicality in the image, and use this verbalization as an input to a better reasoner, namely a large language model. We test our methods on the action-reason statement retrieval task from an advertisements dataset. We show that our verbalization of atypicality achieves stronger results than vision-language models directly predicting the action-reason statements, and better than large language models which use a verbalization not aiming to capture atypicality or unusualness. 
      % \keywords{Visual persuasion \and Visual reasoning \and Atypicality}
\end{abstract}




==> sections/ECCV_dumps/intro1.tex <==
% OUTLINE: 
% PARAPGRAH1: 
%   Advertisement images
%   Why is understanding advertisement images important? And why is it challenging? 
%   
% PARAGRAPH2: 
%   What is atypicality? Why is it important? How is it useful for understanding images? (provide examples?)
%   Previous Works on Atypicality? Their limitations? Why their limitations are important?  
%  IMPORTANT PAPERS TO CITE:  KAREN (A-R TASK), Meiqi (ATPYICALITY DETECTION)
%  PARAGRAPH3: (ATYPICALITY DETECTION)
%       What are we doing in this project? 
%       Advantages compare to the previous works? 
%       Explain our method
%  PARAGRAPH4: (ACTION-REASON DETECTION)
%   How we use atypicality detection for A-R task
%   What is the novelty here? 
%   What is the impact? 
%   What is the contribution? 



% NOVELTIES/CONTRIBUTIONS FOCUS ON IN THIS PROJECT: 

%  First work to see Action-Reason detection Through Atypicality. 
%  (NEW TASK) ATYPICALITY CLASSIFICATION. FIRST WORK TO DO MULTI_LABEL ATYPICALITY CLASSIFICATION ( previous work: binary classification). I was previously infeasible to do ATPYICALITY CLASSIFCIATION. We belive VLM/LLM enables this.
% We tried different ways  of Combining VLM/LLMs
%  DIFFERENT TASKS (ATYPICALITY): 
%   ATYPICALITY MUTLTI_LABEL classification
%   ATYPICALITY STMT CLASSIFICATION
%   FIRST/SECOND OBJECT CLASSIFICATION

% FINDINGS
%   Smaller models are not able to get/understand atypcality
%   VLMs do not have the reasoning power to get atpyicality very well. or connecting them for A-R task



\section{Introduction}

\label{sec:intro}
% \textbf{Things to discuss in order}
% \begin{enumerate}
    % \item  A brief introduction of the task. Why is this task (common sense reasoning) important? Why is it challenging? What is Atypicality? And how we think it will help? 
    % \item Prior works briefly and what they are missing
    % \item our proposed approach. Why LLM/ ChainOfThought Reasoning is helpful? (Do not discuss the hard negative generation)
    % \item Briefly mention our experimental results
% \end{enumerate}

    
    Visual media (e.g., advertisement) content creators may intentionally utilize visual rhetoric\footnote{A rhetorical figure is an artful deviation, relative to audience expectation, that conforms to a template independent of the specifics of the occasion where it occurs\cite{mcquarrie1999visual}} to attract user attention and convey their message \cite{mcquarrie1999visual,guo2021detecting}. Visual rhetoric often includes unique and atypical portrayals of objects, making understanding such atypicality essential to decoding the underlying message and understanding the persuasiveness of visual media \cite{cite}. However, understanding the atypicality and rhetoric of visual media requires a deep understanding of visual contents, such as objects, relationships among objects, and image context. Additionally, often possessing external background knowledge, such as the potential health implications of soda consumption, could facilitate revealing the hidden message of the visual media. \textbf{For example, in Fig.~\ref{fig:intro_examples}, Knowing that rotten teeth are often black, in addition to the relationship between oral hygiene and heart diseases, can aid in decoding the underlying message of the image}. However, unlike humans, computer vision (CV) models struggle to decode visual media's underlying message due to the lack of deep understanding of images and external knowledge. 
    
    \input{figures/intro_examples_plot}
     % However, detecting this type of atypicality is challenging for computer vision models because they may involve metaphorical object transformations or involve creative or unconventional portrayal of objects that require complicated reasoning and commonsense knowledge to decode \cite{guo2021detecting}. 

     Recently, researchers have begun to delve into the understanding of advertisement content, with Visual Commonsense Reasoning (VCR) emerging as a promising approach to evaluate the comprehension capabilities of computer vision (CV) methods. \cite{yeinterpreting,hussain2017automatic} introduced the innovative task of action-reason detection, which entails identifying and interpreting the actions that advertisements suggest to viewers (i.e., What should I do?), along with the rationale for these suggested actions (i.e., Why should I do it?).\textbf{ For instance, in Fig~\ref{fig:intro_examples}, the interpretation 'I should buy this potato chips' coupled with the reason 'Because it is spicy' exemplify responses to these questions, respectively. In this image, the reason is inferred from the atypicality that shows the potato chips is as hot as fire flames.} The concept of atypicality also garnered attention due to its importance in understanding visual persuasiveness and rhetoric of visual media \cite{guo2021detecting}. Existing works in this domain solely focus on predicting whether an advertisement image is atypical or not \cite{guo2021detecting,zhao2017watch}. For example, \cite{guo2021detecting} proposed a self-supervised attention-based method to capture object-level spatial relation and contextual compatibility for the atypicality binary classification task. Indeed, Detecting and differentiating various types of atypicality is an intricate task for intelligent systems, as atypicality often involves diverse and creative metaphorical object transformation detecting this type of atypicality is challenging for intelligent systems. Moreover, a commonsense reasoning capability may be required to understand what kind of atypicality is utilized in the image. However, a lack of common reasoning and a deep understanding of visual contents made identifying different types of atypicality infeasible. However, fortunately, recent vision-language models (VLMs) \cite{liu2023visual,li2023blip,2023GPT4VisionSC} and large-language models (LLMs) \cite{touvron2023llama} have shown strong visual understanding and common reasoning capabilities, opening new possibilities in understanding rhetorical visual media data. 
     
    In this paper, we propose to study the impact of atypicality in understanding advertisement images through the action-reason detection task. Concretely, \textit{we hypothesize that a deeper understanding of atypicality could significantly enhance the accuracy of action-reason detection tasks.} By recognizing and interpreting atypical features within advertisements, CV models may achieve a higher performance level, mirroring a more nuanced human-like comprehension of advertisement content. In fact, as demonstrated in Fig.~\ref{plot:intro_motivation}, we observe that simply utilizing the atypicality ground truth can consistently enhance the performance of current state-of-the-art vision-language models for the action-reason detection task. Motivated by this observation, we propose exploring the understanding of VLMs and LLMs for rhetoric visual media, specifically atypicality. 

     To this aim, we first introduce three tasks of \textit{multi-label atypicality classification, atypicality statement detection, and first-second concept atypical classifications}. We discover that VLMs, especially smaller models, fail to extract atypical information directly from the image effectively as it requires complex multi-step reasoning capabilities. VLMs generally have lower reasoning potential than LLMs. Hence, we propose and compare different methods to verbalize the image and then use an LLM to detect the atpyicality. We discover that while simply \textit{describing the image} can provide complementary to \textit{unusual knowledge extraction} (i.e., \textit{What is unusual about this image? }), this information may be noisy, especially in smaller models. Hence, we incorporate an LLM-based approach (i.e. combine-refine) to combine and summarize all these different information by removing the noisy details, resulting in \textbf{X} and \textbf{Y} improvement on multi-label classification and statement detection tasks. Furthermore, \textbf{TODO: 1st/2nd object classification}.

    % Finally, we utilize our findings in the previous step in the action reason detection task. Introduced by \cite{yeinterpreting, hussain2017automatic}, action reason detection is the task of interpreting advertisement images as intended by designers. The interpretation of each image, contains two parts: action, and reason. The action part is what the designers wants to convince audience to do, and the reason part is why the audience should take that action according to the image. In this task the model is provided with set of options and it must retrieve the correct one based on the input image. In the original dataset, the incorrect options were collected from the annotations of the other images which results in visual difference between the correct and incorrect options and makes it easier for computer vision models to retrieve the correct one. To make this task more challenging for computer vision models, we utilized GPT4 \cite{GPT4} api to generate incorrect options that are semantically different from correct options instead of visually. For example, in one type of incorrect options, we prompted GPT4 to generate incorrect option given the correct option changing an adjective in the correct option to change the meaning of the sentence. This way, while keeping the same visual information, we generated incorrect options.

    
    
To summarize, our contributions are: 
\begin{itemize}
    \item  First to evaluate performance of models on action-reason detection through atypicality
    \item first to use LLM/VLM on this task
    \item Introducing three novel atypicality tasks.    
    \item Proposing a method to generate atypicality-aware verbalization
    \item compare different ways of extracting atypicality and exploring the impact of atypicality for action-reason detection.
    \item  we are hoping our work opens a new door to research and better understanding of persuasive rhetoric images. 
\end{itemize}


==> sections/ECCV_dumps/intro2.tex <==
% \documentclass{article}
% \usepackage{graphicx} % Required for including images
% \usepackage{multirow}
% % \begin{document}


\section{Introduction}

\label{sec:intro}
% \textbf{Things to discuss in order}
% \begin{enumerate}
    % \item  A brief introduction of the task. Why is this task (common sense reasoning) important? Why is it challenging? What is Atypicality? And how we think it will help? 
    % \item Prior works briefly and what they are missing
    % \item our proposed approach. Why LLM/ ChainOfThought Reasoning is helpful? (Do not discuss the hard negative generation)
    % \item Briefly mention our experimental results
% \end{enumerate}

In visual media, particularly advertisements, content creators strategically utilize visual rhetoric to attract the audience and convey a specific message indirectly to the user. They intentionally employ artful deviations, showcasing objects in a unique and atypical manner \cite{mcquarrie1999visual,cite-more}. Understanding such atypical portrayals is pivotal for decoding the intended message and the persuasiveness of the visual media \cite{cite}. For instance, in Fig.~\ref{fig:intro_examples}, \textbf{potato chips are depicted as fire flames to metaphorically represent the product's spiciness, inheriting from features associated with the fire flame.} However, atypicality often involves diverse and creative metaphorical object transformation \cite{cite}, presenting significant challenges in detecting and distinguishing various types of atypicality. Overcoming these challenges to detect atypicality successfully requires a comprehensive understanding of visual content and commonsense reasoning capabilities \cite{guo2021detecting}. However, the lack of such abilities has been a major obstacle to the usability of CV methods for effectively detecting atypicality and incorporating this information for interpreting visual rhetoric. 

Fortunately, recent vision-language models (VLMs) \cite{liu2023visual,li2023blip,2023GPT4VisionSC} and large-language models (LLMs) \cite{touvron2023llama} have shown strong visual understanding and commonsense reasoning capabilities \cite{li2023blip,2023GPT4VisionSC,cite-some-resonig paper}, opening new possibilities in understanding rhetorical visual media data, particularly atypicality detection. In this paper, we propose to harness the potential of state-of-the-art VLMs and LLMs for understanding visual rhetoric. In particular, we propose to study the impact of atypicality in decoding the correct interpretation of rhetoric media. To this aim, following prior works \cite{hussain2017automatic,yeinterpreting}, we adopt the task of action-reason detection to assess the understanding of visual media. This task entails identifying and interpreting advertisements' actions and the rationale for the suggested action. In other words, an action-reason statement essentially answers "What should I do?" and "Why Should I do it?" respectively. Concretely, \textit{we hypothesize that a deep understanding of atypicality will improve the model performance in action-reason detection task}. In fact, as demonstrated in Fig.~\ref{plot:intro_motivation}, we observe that simply utilizing the atypicality annotation can consistently enhance the performance of current state-of-the-art vision-language models for the action-reason detection task.

    \input{figures/intro_examples_plot}

Motivated by the above observation and the promising performance of VLMs and LLMs in various tasks and their strong reasoning capabilities, we first propose to explore and asses recent VLMs' and LLM's understanding of atypicality and whether they can distinguish between different types of atypicality. Secondly, we extend our findings in the first step to design an efficient method to detect and leverage atypicality for enhancing visual rhetoric (i.e. action-reason) understanding. While atypicality is one of the core concepts in visual rhetoric, due to the existing challenges, it remains heavily understudied. In fact, existing studies \cite{guo2021detecting,zhao2017watch} primarily focus on binary classification, oversimplifying the nuanced and multifaceted nature of atypicality in visual media.

Following this premise, we propose three novel tasks: multi-label atypicality classification, atypicality statement detection, and atypical object recognition. As demonstrated in Sec.~\ref{sec:results}, we discover that while VLMs, especially smaller public models, can extract useful information from the image for both atypicality detection and action-reason detection tasks, they fail to infer atypicality directly from the image. This can originate in the lower reasoning potential of current VLMs compared to LLMs \cite{yang2023enhance,cite-to-support-this}. Hence, we propose a novel approach to retrieve informative information from the image by using a VLM (i.e., LLava \cite{liu2023visual}) to verbalize the image and then use an LLM with strong reasoning ability (i.e., GPT-4) for multi-label classification and atypicality statement detection tasks.

Finally, we utilize our findings in the previous step to predict the atpyicality utilized in the advertisement image to devise a corresponding atypicality statement, which will be used as an intermediate link between VLM's output and LLM's input for action-reason detection. VLMs are usually able to generate detailed description of objects in an image; however, due to the lack of knowledge of atypicality, they fail in describing the atypical objects and the relation among them. In this work to address this gap,  we add the detected atypicality statement to the VLM's output before feeding it into the LLM for a comprehensive understanding.

\textbf{TODO: summarize results}

We conduct experiments on three tasks of multi-label classification, atypicality statement detection, and atypical object recognition, as well as action reason detection on the PittAd dataset \cite{hussain2017automatic}. We observe ...
To summarize, our contributions are: 
\begin{itemize}
    \item  First to evaluate the performance of models on action-reason detection through atypicality
    \item first to use LLM/VLM on this task
    \item Introducing three novel atypicality tasks.    
    \item Proposing a method to generate atypicality-aware verbalization
    \item compare different ways of extracting atypicality and exploring the impact of atypicality for action-reason detection.
    \item we utilize GPT-4 to generate semantically hard negatives for action-reason detection task
    \item  we are hoping our work opens a new door to research and better understanding of persuasive rhetoric images. 
\end{itemize}


% \end{document}

==> sections/ECCV_dumps/intro3.tex <==
\section{Introduction}
\label{sec:intro}

In visual media, particularly advertisements, content creators strategically utilize visual rhetoric to attract the audience and convey a specific message in a creative, memorable, and powerful way.
They intentionally employ artful deviations from realism, showing objects in a unique and atypical manner \cite{mcquarrie1999visual}. Understanding such atypical portrayals is pivotal for decoding the intended messages of visual media \cite{williamson1978decoding}. For instance, in Fig.~\ref{fig:intro_examples} (a), the word box appears like tape to denote silencing someone, and in (d), potato chips are depicted as flames to metaphorically represent the product's spiciness, inheriting properties from fire (hotness, with heat metaphorically denoting flavor). Because atypicality often involves diverse and creative metaphorical object transformations \cite{williamson1978decoding,yeinterpreting}, it is challenging for classic neural computer vision systems to (1) recognize the objects and their relation despite their unusual appearance, and (2) interpret what this atypicality means, in terms of the message the ad wants to convey.  

Recent vision-language models (VLMs) \cite{liu2023visual,li2023blip,2023GPT4VisionSC} 
%and large-language models (LLMs) \cite{touvron2023llama} 
have shown strong visual understanding capabilities \cite{li2023blip,2023GPT4VisionSC}, opening new possibilities in understanding persuasive visual media, particularly atypicality. 
However, while they achieve strong object recognition results \cite{NEURIPS2023_761c3284} and decent reasoning \cite{liu2023visual}, we find their reasoning skills are worse than ``blind'' large language models. 
Thus, we experiment with different verbalization strategies to convey relevant information about the ads, including atypicality, to language models which then reason about these ads. 

In particular, we study the impact of atypicality in decoding the persuasive messages of advertisements, using the action-reason retrieval task proposed in \cite{hussain2017automatic,yeinterpreting}. This task entails identifying and interpreting advertisement's actions and the rationale that the ad provides for taking the suggested action. In other words, an action-reason statement answers ``What should I do based on this ad?'' (e.g., buy these chips) and ``Why should I do it, based on the ad?'' (e.g., because they are spicy). \textit{We hypothesize that a deep understanding of atypicality will improve the model performance in action-reason matching/retrieval}. As a proof of concept, in Fig.~\ref{plot:intro_motivation} we demonstrate that an oracle using the atypicality annotation can consistently enhance the performance of current state-of-the-art vision-language models for action-reason retrieval.
In practice, to boost the reasoning capacity of our proposed method, we tap into large language models by first extracting relevant information about content and atypicality in the ad using a VLM, then querying an LLM using this verbalization of the image. 

\input{figures/intro_examples_plot}

Existing studies of atypicality \cite{guo2021detecting,zhao2017watch} focus on binary classification, oversimplifying the nuanced and multifaceted nature of atypicality in visual media. Instead, we study atypicality understanding using three distinct and novel tasks: multi-label atypicality classification, atypicality statement retrieval, and atypical object recognition. As demonstrated in Sec.~\ref{sec:results}, we discover that VLMs (even smaller public models) can extract useful information from the image, which can be used for both atypicality recognition and action-reason retrieval tasks. However, they achieve suboptimal results in inferring atypicality or reasoning about action-reason directly from the image. This can originate in the lower reasoning potential of current VLMs compared to LLMs \cite{yang2023enhance}. Hence, we propose a novel approach to retrieve informative information from the image by using a VLM (i.e., LLaVA \cite{liu2023visual}) to verbalize the image and then use an LLM with strong reasoning ability (i.e., GPT-4) for multi-label classification and atypicality statement retrieval.
Finally, we utilize the atypicality statement as an intermediate link between the VLM's output and LLM's input.
We conduct extensive experiments on the PittAds dataset \cite{hussain2017automatic} and demonstrate the benefit of atypicality-aware verbalization to LLMs for persuasive image reasoning.

To summarize, our contributions are as follows: 
\begin{enumerate}[nolistsep,noitemsep]
    \item We are the first to evaluate the models on action-reason retrieval through atypicality inference and the first to use LLMs/VLMs for this task.
    \item We introduce three novel atypicality tasks.    
    \item We propose atypicality-aware verbalization for persuasive images.
    \item We test different ways of extracting atypicality for action-reason retrieval.
    \item We utilize GPT-4 to generate %semantically 
    hard negatives for action-reason retrieval.
    %\item  we are hoping our work opens a new door to research and better understanding of persuasive rhetoric images. 
\end{enumerate}


==> sections/ECCV_dumps/method.tex <==
\section{Methodology}
\label{sec:method}

Deciphering the unique and uncommon relationships among objects is essential for interpreting the intent behind visual media designs. 
% Conventional CV methods struggle due to the intricate common sense reasoning and extensive external knowledge required to identify and distinguish various atypicalities. 
We 
%follow the action-reason retrieval framework defined in \cite{ye2018advise,yeinterpreting} and 
use the atypicality annotations from \cite{yeinterpreting}, but our approach is dramatically different as we propose harnessing off-the-shelf VLMs and LLMs for atypicality understanding and the action-reason retrieval tasks without additional model training (i.e., zero-shot). 
The key novelty is formulating a verbalization of the image using an off-the-shelf VLM, which is fed to an LLM to get a description of the atypicality in the image. Both are used again to prompt an LLM for the appropriate action-reason statement, which serves as a decoding of the ad's message. 

\input{figures/tasks}

While \cite{yeinterpreting} defined eight types of atypicality, the only prior works training models for atypicality \cite{yeinterpreting,guo2021detecting} only explore the binary task (predict if an image is typical or atypical) due to the challenge of the task of classic neural computer vision methods (CNNs and transformers). We propose a framework piping outputs of modern VLMs to LLMs to enable new useful atypicality tasks. We aim for a more comprehensive understanding of atypicality, to provide context for action-reason understanding (i.e., what action the ad prompts the viewer to do, and what reasons it provides for taking the suggested action). To build towards this understanding, we first propose a new Multi-label Atypicality Classification (MAC) task. Since this task only provides a label, we next tap into the additional atypicality annotations provided by \cite{yeinterpreting}, which name the objects involved in the atypical portrayal (e.g., The surface of the \underline{bottle} mimics the texture of \underline{feather}, as shown in Fig.~\ref{fig:tasks}). 
%We experiment with different ways to combine VLMs and LLMs to enable zero-shot retrieval of an atypicality statement naming both objects involved in the atypicality and their relation. 
We name this task Atypicality Statement Retrieval (ASR). 
To explore the visual reasoning of VLMs further, we also provide results on a new Atypical Object Recognition (AOR) task. 
Our analysis reveals that, although VLMs initially struggle to perform MAC and ASR directly, they show a promising capability to extract informative insights about the atypical aspects of images which was then fed into an LLM for the final task outputs.
%We test various prompting strategies to verbalize the image to be utilized by an LLM classifier for atypicality understanding tasks, as explained in Sec.~\ref{sec:proposed-approach}. 
%Lastly, we tackle our primary objective: \textit{enhancing action-reason retrieval performance by detecting and incorporating atypicality.} 
Concretely, we leverage a prompt \textit{UH: What is unusual about this image?} to extract and detect atypicality from the image, which will be incorporated for action-reason retrieval tasks. However, while atypicality adds depth to the manifest content of advertisement images, it complements visually explicit elements such as objects, relations among objects, scene description, and scene-text. Thus, we propose constructing the final textual atypicality-aware verbalization by combining the \textit{$UH$} with more surface-level content. 
%The final verbalization will be then used for action-reason retrieval (Sec.~\ref{sec:proposed-approach}). In practice, we use LLaVA, a sota VLM, for atypicality-aware verbalization $\mathcal{T}_{\mathcal{V}}$ of the image $I$. $\mathcal{T}_{\mathcal{V}}$ will be used by a powerful LLM like GPT-4 to significantly enhance the understanding of atypicality understanding and action-reason retrieval tasks. 
% PittAd dataset  \cite{hussain2017automatic,yeinterpreting} is utilized in this work since it is publicly available and contains required ground-truth atypicality and action-reason annotations. 
% Fig.~\ref{fig:form-overview} shows the overview of our proposed model.

\input{figures/atyp_def_rel}

\subsection{Established Atypicality Understanding Tasks}
\label{sec:atyp-tasks}

Ye et al. \cite{yeinterpreting} devised a taxonomy of atypicality based on object transformations. In this work, we focus on the subset of atypicality categories that all entail two objects (examples in Fig~\ref{fig:intro_examples}): (1) Texture Replacement 1 (TR1): Objects’ texture borrowed from another object, (2) Texture Replacement 2 (TR2): Texture created by combining several small objects, Object Inside Object (OIO):  An object is completely or partially inside of another object, and (4) Object Replacement (OR): The whole object appearing in the context normally associated with another.
We define the following new atypicality understanding tasks. 

\textbf{Multi-label Atypicality Classification (MAC).} 
Unlike prior works \cite{yeinterpreting,guo2021detecting} that only address the presence of atypicality, we formulate atypicality detection as a multi-label classification task. The PittAds dataset provides three annotations of atypicality per image (from three different annotators) that may not be of the same type. For instance, Fig.~\ref{fig:intro_examples} (c) can be classified as `Object Inside Object' (Earth inside of a cup sleeve) and `Object Replacement' (Earth replaces coffee cup). 
The labels provided by one or two of the three annotators may include `Not Atypical' (NA) in addition to the four atypicality categories, suggesting the image is typical. 
%MAC demands a comprehensive analysis to categorize the image into fine-grained atypicality categories. 
The complexity of differentiating between the atypicality categories $\mathcal{A}$ requires more comprehensive and clear definitions $\mathcal{D}_{\mathcal{A}}$ than provided by \cite{yeinterpreting}. We create and show these in Fig.~\ref{fig:atyp_def_stmt}: they not only distinguish different atypicality categories but also provide a hint of how the atypicality impacts the interpretation of the image (e.g., Fig.~\ref{fig:intro_examples} (e) is an example of TR1, the texture of beer is replaced by feather to advertise the lightness of the beer borrowed from the feather). 
MAC challenges the VLMs/LLMs tested to predict the applicable atypicality categories $a \in \mathcal{A}$ for each image $I$ (see supp for prompts).

\input{figures/method_model_figure}
% \noindent
\textbf{Atyplicality Statement Retrieval (ASR).}
We formulate atypicality inference as retrieval of a relation between two objects. We represent atypicality $\mathcal{A}$ by templates $\mathcal{S_{\mathcal{A}}}$ according to the definitions in Fig.~\ref{fig:atyp_def_stmt}.
A statement $s$ is a triplet $s = (a, o^p, o^s)$. The $o^p$ and $o^s$ are described in Sec. 3.6 of the PittAds dataset \cite{yeinterpreting}. For TR1 and TR2, $o^p$ is the object that has a new texture, and $o^s$ is the source of this texture. For OIO, $o^p$ is the object on the inside, and $o^s$ on the outside. For OR, $o^p$ is the object placed in the context of another, and $o^s$ is the expected object. 
The relation $r$ is fixed based on the atypicality category. 
%Examples are shown in Fig.~\ref{fig:intro_examples}.
Given an advertisement $I$, the ASR task involves distinguishing the correct atypicality statement ${s}^{+}$, which accurately reflects the atypical relationship, from negative statements $\{\Bar{s_{i}}\} \in {S}^{-}$. 
These negatives ${S}^{-}$ are automatically generated for a pos. statement $s^{+} = (a^+,o^{+p},o^{+s})$ by (1) \textbf{Wrong object}: We retrieve the objects from $K$ random images in the datasets (i.e, $I_k=(a_k, o^{p}_{k}, o^{s}_{k})$ where $k = 1 $ to $K$) to create $2K$ negatives by replacing the $o^{+p}$ and $o^{+s}$ (e.g., $\Bar{s}_1 = (a^+, o^{p}_{1}, o^{s}_{1})$ and $\Bar{s}_2 = (a^+, o^{s}_{1}, o^{p}_{1})$); 
(2) \textbf{Wrong atypicality relation}: We keep the original objects but change the relation with one not in the ground-truth, to create a maximum of 3 negatives (i.e., $(\Bar{a}_i, o^{+p}, o^{+s})$); and (3) \textbf{Swapped primary/secondary objects}: we create $(a^+,o^{+s},o^{+p})$ to examine the deep understanding of the model about the relation between the objects. ASR thus requires the model to understand the objects and atypicality relation, and differentiate between primary and secondary objects. ASR can be directly employed in the final method to detect the atypicality statement for enhancing action-reason retrieval, bridging the gap between MAC and action-reason retrieval. We select $K=2$.

% \noindent
\textbf{Atypical Object Recognition (AOR).}
To assess the fine-grained visual understanding of VLMs, we introduce the task of recognizing the primary and secondary objects in the atypical image. Given ad image $I$ and atypicality statement $s = (a^{+}, -, -)$ where true atypicality $a^{+}$ without the primary/secondary objects (i.e., $-$) is fed to the model, the goal is to assess the ability of the model to generate the correct primary/secondary objects. AOR can be considered as a fill-in-the-blank task based on the ASR templates $\mathcal{S}_{\mathcal{A}}$. 

\subsection{Proposed Approach} 
\label{sec:proposed-approach}

% We believe that the current VLMs' limitations in commonsense reasoning hinder their ability to directly address atypicality detection and action-reason retrieval tasks. Therefore, we propose to use an LLM, which has shown strong reasoning ability for the final downstream task. However, since LLMs such as GPT-4 cannot process images directly, we use LLaVA to produce an effective verbalization $\mathcal{T}_\mathcal{V}$ that can be successfully used for atypicality understanding tasks and the subsequent action-reason retrieval. 

The proposed method for action-reason retrieval (Fig.~\ref{fig:method-overview}) consists of three steps. (i) Atypicality-aware image verbalization: We use LLaVA \cite{liu2023visual} and GPT-4 \cite{achiam2023gpt} to generate an explicit verbalization $\mathcal{T}_{\mathcal{V}}$ that includes information about the atypicality in the image; (ii) Atypicality statement retrieval: We use GPT-4 to retrieve the atypicality statement $\hat{s}=(\hat{a}, \hat{o}^p, \hat{o}^s)$. (iii) Action-reason retrieval: GPT-4 uses the combination of (i) and (ii) to retrieve final action-reason statement. 

% \noindent
\textbf{(i) Atypicality-aware image verbalization.}  Each ad image $I=\left(V, T\right)$ is composed of visual content ($V$) (i.e., list of objects) and textual content ($T$) (i.e., scene-text). We obtain $V$ and $T$ by querying LLaVA for up to 5 objects and a list of textual information visible in the image. However, this information is not sufficient to fully comprehend the image. Hence, we additionally prompt LLaVA with
(1) $ImageNarration$ ($IN$): LLaVA's responses when prompted \textit{Describe the image in detail.} (2) $UnusualHighlighter$ ($UH$): LLaVA's reponse when asked \textit{What is unusual about the image?} The results on MAC (Table~\ref{tab:MAC_ASR_Full_set}) show that $UH$ is very effective in understanding the unusualness of the image, which is closely related to the atypicality, while $IN$ could be used to retrieve the atypicality statement $\hat{s}$ as it provides more information about the scene and the objects. Thus, to construct the final description $\mathcal{T}_{\mathcal{V}}$, we propose combine unusualness (i.e., $UH$) with objects $V$, scene-text $T$, and image description ($IN$). We leverage an LLM to combine all this information in a monolithic manner. 
%$\mathcal{T}_{\mathcal{V}}$ will be further exploited to detect the action-reason statements. 

% \noindent
\textbf{(ii) Atypicality Statement Retrieval.}
To retrieve the atypicality statement, we construct the possible statements. Option Generator (teal module in Fig~\ref{fig:method_asd}) combines $V$ and $\mathcal{S}_{\mathcal{A}}$ to create all possible statements ${S}_I$. Specifically, each pair of objects $(o_i,o_j)$ will be combined with atypicality statement templates $s \in \mathcal{S}_{\mathcal{A}}$ to create atypicality statements $(a_k, o_i/o_j, o_j/o_i)$ for all $a_k \in \mathcal{A}$. Next, we pass these atypical statements ${S}_I$ along with verbalized description $\mathcal{T}_{\mathcal{V}}$ into an LLM to retrieve the most accurate atypicality statement $\hat{s}$.

% \noindent
\textbf{(iii) Action-Reason Retrieval (ARR).} 
%Finally, we can address the end goal task (i.e., action-reason retrieval).
\cite{hussain2017automatic} provided three action-reason statements for each image. These action-reason statements may have different plausible reasons for the same action. Therefore, given three plausible (i.e., positive) and many implausible (i.e., negative) action-reason statements, the task is to detect all of the plausible action-reason statements $\{\hat{ar}_I \}_{i=1}^3$. 
We proposed different verbalization variants, including concatenation and LLM-based combination (i.e. $\mathcal{T}_{\mathcal{V}}$) of $V, T, IN, UH$, as well as concatenation of $\hat{s}$ with $\mathcal{T}_{\mathcal{V}}$, to be leveraged by an LLM %GPT-4 
to retrieve the final action-reason statement. %Furthermore, to demonstrate that our approach is capable of a deep understanding of the image, we leveraged an LLM to produce \textbf{semantically hard negatives} (Sec.~\ref{sec:exp_setup}).











==> tables/ASR_error_analysis.tex <==
\setlength{\tabcolsep}{0.5pt}

\begin{table}[!tp]
% \vspace{-0.67cm}
\centering
%is based on $UH$. LLaVA + GPT-4 verbalization. 
%, $\hat{s}_{UH}$: atypc prediction based on UH}
\scriptsize
\begin{tabular}{lc||c|c|c|c}
\toprule

 \tiny{classifier} & \tiny{Verb.} & \tiny{Wrong Object} & \tiny{Swap Primary/Secondary object} & \tiny{Wrong Relation} & \tiny{Total}\\
\hline
\hline
LLaVA& $I$&  83 & 156   & 709 & 948\\
 \hline
\multirow{2}{*}{GPT-4} &$IN$&67 &323 & 101 & 491\\
 &$UH$&56 &306 & 139 &501\\
% \vspace{-0.1cm}
\bottomrule
\end{tabular}
% \vspace{-0.5cm}
\caption{{\textbf{Error Analysis of ASR on full-set.} Number of errors per type of ASR negative option.}
}
\label{tab:ASR_error_analysis}
\end{table}

==> tables/ECCV_dump/action_reason_small_set.tex <==

%  final table

\begin{table*}[!tp]\centering

\scriptsize
\begin{tabular}{lc||ccc|ccc|c}\toprule

&& \multicolumn{6}{c|}{\textbf{\textit{Multi}}} & \textbf{\textit{Single}}\\

\textbf{Model}&\textbf{Verb.}& \multicolumn{3}{c|}{\textbf{\textit{Precision@k}}} & \multicolumn{3}{c|}{\textbf{\textit{Top-k Acc}}}& \\
&&\textbf{k=1} &\textbf{k=2} &\textbf{k=3} &\textbf{k=1} &\textbf{k=2} &\textbf{k=3} & \textbf{Acc} \\
\hline
\hline
% CLIP & $I$ & 64.52 &34.48 & 22.98 & 20.97& 47.18 &64.52 & 20.97 \\
% CLIP (KAFA) &$I +T$& 47.18 & 25.40 & 16.94 & 15.73 & 32.26  & 47.18 & 15.73 \\
% \hline
% LLaVA &$I$ &\textbf{59.67} &\textbf{38.27} &26.06 &32.92 & 48.14&\textbf{59.67} &26.00 \\
% % BLIP-2 &$I$ &Failed &Failed &Failed &Failed &Failed &Failed &37.38 \\
% % MiniGPT4 &$I$ & & & & & & & \\
% GPT-4V &$I$ &56.40 &38.00 &\textbf{26.80} &22.00 & \textbf{49.60} &56.40 &\textbf{90.37} \\

% \hline

\multirow{3}{*}{Vicuna} 
&$V + T$ &64.11 & 41.53 & 27.69 & 24.19 &45.56 & 64.11   & 44.35\\
&$IN$ & 64.92 & 43.55 & 29.17 & \textbf{24.60} & 43.55 & 64.92 & 45.56\\
&$UH$ & 60.89 & 38.71&  25.94 & 20.97 & 40.32 & 60.89 & 37.90\\
\hline
& $V + T + IN + UH$ & 69.35 & 45.33 & 30.88 & 23.80 & 45.21 & 69.35 & 48.39 \\

% small: &$V + T + IN + UH$ & 71.37 & \textbf{47.58} & \textbf{32.12} & \textbf{27.42} & \textbf{48.39 }& 71.37 & 48.39\\

\multirow{2}{*}{Ours (Vicuna)} &$\mathcal{T}_\mathcal{V} \setminus UH$ & 69.35 &  44.35 & 29.57 & 22.98 & 45.56 & 69.35 & 48.39 \\


&$\mathcal{T}_\mathcal{V}$ &71.37 & \textbf{46.77} & 31.45 & 23.39 & 45.16 & 71.37 & 46.37\\
 

    &$\mathcal{T}_\mathcal{V}+\hat{s}_{IN}$ & \textbf{71.77} &\textbf{ 46.77} & \textbf{31.59} & 23.79 & \textbf{46.77} & \textbf{71.77} & \textbf{48.79}\\
 
 % &$\mathcal{T}_\mathcal{V} + \hat{s}_{IN}$ &68.32 & 44.52 &30.25&22.95& 43.24 & 68.32 \\


% \multirow{2}{*}{Ours(Vicuna) with GPT4 verb} &$\mathcal{T}_\mathcal{V}$ &\textbf{72.18} & \textbf{47.18} &31.99 &28.23 &48.39 & \textbf{72.18} & \textbf{48.39 }\\
% &$\mathcal{T}_\mathcal{V} + \hat{s}_{UH}$ &  71.37 & \textbf{47.18} &\textbf{ 32.12 }& \textbf{29.44} & \textbf{48.79} & 71.37 &  47.98\\

% &$\mathcal{T}_\mathcal{V} + \hat{s}_{\mathcal{T}_\mathcal{V}}$ & 71.77 & 46.77 & 31.59 & 27.82 & \textbf{48.39} & 71.77 & \textbf{48.39} \\

\hline
\hline

\multirow{4}{*}{GPT-3.5} &$V + T$ &85.43 &59.51 &40.62 &46.56 &68.02 &85.43 
& 72.46 \\ %&91.50 \\
&$IN$ & 89.07& 64.78&  45.48 & \textbf{65.99} & 79.76 & 89.07 & 77.41 
 \\  %& \textbf{91.90} \\
&$UH$ & 84.62& 58.91& 40.89 & 52.63 &70.45 & 84.62 & 76.61 \\ %&&89.88 \\

\hline

&$V+T+IN+UH$ &90.32 &64.92 &45.43 &48.39 &74.60 & 90.32 &  74.39 \\ %&90.32 \\


\multirow{2}{*}{Ours (GPT-3.5)} &$\mathcal{T}_\mathcal{V} \setminus UH$ & 91.09 & 66.81 & 46.55 & 62.75 & 78.94 & 91.09 & 78.54 \\ %&78.86\\ 

&$\mathcal{T}_\mathcal{V}$ &\textbf{91.90} & \textbf{67.61} & \textbf{46.96} & 63.15 & 79.75 & \textbf{91.90} & \textbf{78.94 }\\ %&& 78.13\\
 &$\mathcal{T}_\mathcal{V} + \hat{s}_{IN}$ & \textbf{91.90} & 67.20 & 46.69 & \textbf{65.99} & \textbf{81.78} & \textbf{91.90} &  72.87 \\ %74.38 \\ %&\\


% \multirow{3}{*}{Ours(GPT 3.5) + GPT4 verb}&$\mathcal{T}_\mathcal{V}$ &90.28 &\textbf{ 65.38} & \textbf{45.61} &\textbf{ 68.42 }& 72.87 &90.28 & \textbf{92.31} \\
% &$\mathcal{T}_\mathcal{V} + \hat{s}_{UH}$ &89.43 &63.82 &44.31 &64.63 & 70.37 &89.43 &91.90 \\

% &$\mathcal{T}_\mathcal{V} + \hat{s}_{\mathcal{T}_\mathcal{V}}$& \textbf{90.65} &64.23 &44.72 &65.85 &71.66 &\textbf{ 90.65} &91.90 \\


\hline
\hline

\multirow{4}{*}{GPT-4} &$V + T $&92.71 &84.62 &72.47 &84.55 & 89.52 &92.71 &95.55 \\
&$IN$ & 89.92& 78.23& 64.65&77.42 &85.08 & 89.92&93.88 \\
&$UH$ & 80.41& 63.67 & 50.48&62.04 &72.65 & 80.41&95.08 \\

\hline


&$V+T+IN+UH$ &96.37 &86.49 &72.45 &72.18 &89.11 &96.37 &96.37 \\

\multirow{3}{*}{Ours (GPT-4)} &$ \mathcal{T}_{\mathcal{V}} \setminus UH$ & 94.34 & 85.63& 73.42 & 84.62 & 90.28 & 94.34 & 88.21\\

&$\mathcal{T}_\mathcal{V}$ &96.77 &87.30 &\textbf{74.60} &84.96 &91.46 & 96.77 & \textbf{96.77} \\

% &$\mathcal{T}_\mathcal{V} + \hat{s}_{UH}$&96.76 & \textbf{88.06 }& 74.09 & \textbf{86.64} & 90.69 & 96.76 &96.36 \\

&$\mathcal{T}_\mathcal{V} + \hat{s}_{IN}$ &96.77 &\textbf{87.77} &73.65 &\textbf{87.09} & \textbf{91.54} & 96.77  & 96.36 \\


&$\mathcal{T}_\mathcal{V} + \hat{s}_{\mathcal{T}_\mathcal{V}}$ &\textbf{97.17 }&86.99 &73.55 &85.02 &91.50 & \textbf{97.17} &96.76 \\


\bottomrule
\end{tabular}
\caption{\textbf{ARR on Small-set}. Best result per LLM/column is bolded. `Multi' means we ask the LLM for multiple outputs, `Single' for one.
%LLaVA + GPT-4 Verbalization. Precision@k is un-ranked. $\mathcal{T}_{\mathcal{V}}$: combine, $\hat{s}_{i}$: atypc prediction based on $\hat{s}_{\mathcal{T}_\mathcal{V}}$ or $\hat{s}_{UH}$ with GPT4. 
% The results on the both commercial LLMs show that the verbalization methods that highlight atypicality in the image (i.e. $UH, \mathcal{T}_\mathcal{V}, $)
}
\label{tab:tab_arr_small}
\end{table*}



% %Please add the following packages if necessary:
% %\usepackage{booktabs, multirow} % for borders and merged ranges
% %\usepackage{soul}% for underlines
% %\usepackage[table]{xcolor} % for cell colors
% %\usepackage{changepage,threeparttable} % for wide tables
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% \begin{table}[!htp]\centering
% \caption{\textbf{Multi-label Selection Action Reason Retrieval.} Results on small set. P@1, P@2, and P@3 are unranked precisions.}\label{tab: multi-selection-sample}
% \scriptsize
% \begin{tabular}{l|c|c|c|c}\toprule
% Model &Verb. Method &P@1 &P@2 &P@3 \\\midrule
% \hline
% CLIP(I) & - &59.68  &33.06  &22.04  \\
% CLIP(KAFA) &- &68.95  &38.31  &25.54  \\
% \hline
% LLaVA &- &59.67  &38.27  &26.06  \\
% BLIP-2 &- &0.0&Failed&Failed \\
% MiniGPT4 &- & & & \\
% GPT-4V &- &56.40  &38.00  &26.80  \\
% \hline

% \multirow{6}{*}{Vicuna} &V + T &65.37  &42.14  &28.09  \\
%  &IN & & & \\
%  &UH & & & \\
%  &Combine &70.56  &45.97  &31.72  \\
%  &Combine + pred-atypiclaity (UH) & & & \\
%  &Combine + pred-atypiclaity (combine) & & & \\
% \hline
% \multirow{7}{*}{GPT 3.5} &V + T &85.43  &59.51  &40.62  \\
%  &IN & & & \\
%  &UH & & & \\
%  &\textbf{Combine} &90.28  &\textbf{65.38 } &\textbf{45.61 } \\
%  &Combine + pred-atypiclaity (UH) &89.43  &63.82  &44.31  \\
%  &Combine + pred-atypiclaity (combine) &\textbf{90.65 } &64.23  &44.72  \\
%  &Concat-Simple &90.32  &64.92  &45.43  \\
% \multirow{8}{*}{GPT 4} &V + T &92.71  &84.62  &72.47  \\
%  &IN & & & \\
%  &UH & & & \\
%  &\textbf{Combine} &96.77  &87.30  &\textbf{74.60 } \\
%  &\textbf{Combine + pred-atypiclaity (UH)} &96.76  &\textbf{88.06 } &74.09  \\
%  &\textbf{Combine + pred-atypiclaity (combine)} &\textbf{97.17 } &86.99  &73.55  \\
%  &Combine 2 &95.95  &86.84  &72.33  \\
%  &V + T + IN + UH &96.37  &86.49  &72.45  \\
% \bottomrule
% \end{tabular}
% \end{table}

%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}



% \documentclass{article}
% \usepackage[table, svgnames, dvipsnames]{xcolor}
% \usepackage{makecell, cellspace, caption}
% % \setlength\cellspacetoplimit{3pt}
% % \setlength\cellspacebottomlimit{3pt}
% \begin{document}

% \begin{table}
%         \centering\captionsetup{justification = centering}
%         \caption{Amount of exposure of default towards 3 counterparties\\ (with netting and collateral agreement)}
%         %{\centering}
%         \label{1}
%         \begin{tabular}{|Sc|Sc|Sc|}
%             \hline
%             \rowcolor{Gainsboro!60}
%             Counterparty & \makecell{Amount of EAD\\ (with netting)} & \makecell{Amount of EAD\\ (no netting)}\\
%             \hline
%             A & \phantom{1}\$\,29,637,720 & \phantom{1}\$\,92,604,560 \\
%             B & \phantom{1}\$\,38,250,400 & \$\,107,949,900\\
%             C & \$\,124,619,600 & \$\,124,619,600 \\
%             \hline
%             Total&\$\,192,507,800 & \$\,325,174,100\\
%             \hline
%         \end{tabular}
% \end{table}

% \end{document} 

==> tables/action_reason_full.tex <==
% \begin{adjustwidth}{-4.5 cm}{-4.5 cm}\centering
\begin{table}[!htp]
\centering
\scriptsize
\caption{Comparative accuracy of various models in action reason retrieval on 1168 images sample.}
\label{tab:ar-full}
\begin{tabular}{l|cc}
    \toprule
    Classifier & Method                  & Acc                \\
    \midrule
    % CLIP      & -                       & 54.00\%             \\
    LLaVAt       & -                      &0.00\%             \\ 
    BLIP-2     & -                       & 0.80\%             \\
    CLIP   & -                       & 0.00\%             \\
    \midrule
    FLanT5     & Combine(V,T, IN, UH)    & 0.00\%             \\
    \midrule
    LLama2     & Combine(V,T, IN, UH)    & 0.00\%             \\
    \midrule
    GPT 3.5    & Combine(V,T, IN, UH)    & 0.00\%     \\
    \midrule
    GPT 4      & Combine(V,T, IN, UH)    & 0.00\%            \\
\bottomrule
\end{tabular}
\end{table}
% \end{adjustwidth}

==> tables/action_reason_gpt4v.tex <==

\setlength{\tabcolsep}{0.5pt}


\begin{table}[t]%[tp]
\centering

%$\mathcal{T}_{\mathcal{V}}$: combines $V+T+IN+UH$ using LLM based on GPT-4V verbalization.}

\scriptsize
\begin{tabular}{l||ccc|ccc}\toprule
% \multirow{3}{*}{\textbf{Classifier}}&\multicolumn{6}{c}{\textbf{\textit{Multi}}}  \\ %& \textbf{\textit{Single}}\\

\multirow{2}{*}{\textbf{Classifier}}&  \multicolumn{3}{c}{\textbf{\textit{precision@k}}} & \multicolumn{3}{c}{\textbf{\textit{Top-k acc}}}\\     %&\multirow{2}{*}{\textbf{Acc}} \\
 & \textbf{k=1} &\textbf{k=2 }&\textbf{k=3} &\textbf{k=1} &\textbf{k=2} &\textbf{k=3} \\
\hline
\hline
LLaVA  &59.67 &38.27 &26.06 &32.92 &48.14 &59.67 \\ %&26.00 \\
GPT-4V  &97.17 &89.91 & 74.86 & 77.01 & 90.32 & 97.17 \\ %&90.00\\
GPT-4($\mathcal{T}_\mathcal{V}$ )&\textbf{97.58} &\textbf{90.72} &\textbf{76.61} &\textbf{81.04} &\textbf{92.74} &\textbf{97.58} \\ %&97.90\\
% GPT-4 & $\mathcal{T}_\mathcal{V} + \hat{s}_{\mathcal{T}_\mathcal{V}}$&\textbf{97.97} &90.49 &75.70 &\textbf{81.37} &94.73 &97.97 &0 \\
\bottomrule
\end{tabular}
\caption{\textbf{GPT-4V verb. for $\mathcal{T}_{\mathcal{V}}$ in Multi-ARR on small set}.}
\label{tab:action_reason_gpt4v}
\end{table}

==> tables/action_reason_table_ab.tex <==


% \begin{table}[h]
% \centering

% \caption{Performance of different descriptions on action reason task}
% \begin{tabular}{lcc}
% \hline

% \textbf{Model}                               & \textbf{Accuracy}          \\ \hline
% CLIP                                         & 41.70 \textcolor{red}{(-41.10)} \\ 
% BLIP-2 baseline                              & 82.80                      \\ 
% LLAVA                                        & 26.00 \textcolor{red}{(-56.80)} \\ 
% \hline
% GPT4 with Combine Description                & 90.15 \textcolor{ForestGreen}{(+7.35)} \\ 
% Atypicality Aware GPT4 with Combine Description & 89.80 \textcolor{ForestGreen}{(+7.00)} \\ 

% GPT4 with Combine Refine Description         & 89.09 \textcolor{ForestGreen}{(+6.29)} \\ 
% Atypicality Aware GPT4 with Combine Refine Description & 89.60 \textcolor{ForestGreen}{(+6.80)} \\ 
% GPT4 with Concat Description                 & 83.80 \textcolor{ForestGreen}{(+1.00)} \\ 
% Atypicality Aware GPT4 with Concat Description & -                        \\ 
% GPT4 with Unusual Description                & 85.40 \textcolor{ForestGreen}{(+2.60)} \\ 
% Atypicality Aware GPT4 with Unusual Description & 89.80 \textcolor{ForestGreen}{(+7.00)} \\ 
% GPT4 with Single Step Description            & -                          \\ 
% Atypicality Aware GPT4 with Single Step Description & -                  \\ \hline
% \end{tabular}
% \end{table}

% \begin{adjustwidth}{-4.5 cm}{-4.5 cm}\centering
% \begin{table}[!htp]
% \centering
% \scriptsize
% \caption{Comparative accuracy of various models in action reason detection on 250 images sample.}
% \label{tab:ar-sample}
% \begin{tabular}{l|cc}
%     \toprule
%     Classifier & Method                  & Acc                \\
%     \midrule
%     % CLIP      & -                       & 54.00\%             \\
%     LLaVA       & -                      & 26.00\%             \\ 
%     BLIP-2     & -                       & 82.80\%             \\
%     MINIGPT4   & -                       & 0.00\%             \\
%     \midrule
%     FLanT5     & IN                      & 0.00\%             \\
%                & UH                      & 0.00\%             \\
%                & Concat(V,T, IN, UH)     & 0.00\%             \\
%                & Combine(V,T, IN, UH)    & 0.00\%             \\
%     \midrule
%     Vicuna1.5     & IN                      & 0.00\%             \\
%                & UH                      & 0.00\%             \\
%                & Concat(V,T, IN, UH)     & 0.00\%             \\
%                & Combine(V,T, IN, UH)    & 0.00\%             \\
%     \midrule
%     GPT 3.5    & IN                      & 58.13\%     \\
%                & UH                      & 53.84\%     \\
%                & Concat(V,T, IN, UH) simple     & 61.94\%     \\
%                & Concat(V,T, IN, UH)    & 65.72\%     \\
%                & Combine(V,T, IN, UH)    & 60.32\%     \\
%     \midrule
%     GPT 4      & IN                      & 0.00\%            \\
%                & UH                      & 85.40\%            \\
%                & Concat(V,T, IN, UH)     & 91.90\%            \\
%                & Concat(V,T, IN, UH)    & 88.26\%            \\
%                & Combine(V,T, IN, UH)    & 91.90\%            \\
% \bottomrule
% \end{tabular}
% \end{table}
% % \end{adjustwidth}




==> tables/asr_full.tex <==
% \begin{adjustwidth}{-4.5 cm}{-4.5 cm}\centering
% \begin{table}[!htb]
% \centering
% \scriptsize
% \caption{Comparative accuracies of various models in atypicality statement detection.}
% \label{tab:atyp-stmt}
% \begin{tabular}{lcc}

% \toprule
% {Model} & {Accuracy ()} \\
% \midrule
% CLIP & 54 \\
% LLAVA  & 27 \\
% Multistep Sequential LLAVA & 48.5 \\
% Sequential LLAVA & 29.9 \\
% GPT4v & 35.18 \\
% Multistep Sequential GPT4v & 64.4 \\
% GPT4 with Single Step Description & 61.2 \\
% CoT GPT4 with Single Step Description & 57.7 \\
% GPT4 with Unusual Description & 61.6 \\
% CoT GPT4 with Unusual Description  & 59.68 \\
% \bottomrule
% \end{tabular}
% \end{table}
% \end{adjustwidth}



% \begin{adjustwidth}{-4.5 cm}{-4.5 cm}
% \centering
\begin{table}[!htb]
\centering
\scriptsize
\caption{\textbf{Atypicality Statement Retrieval (ASR).} All results on the smaller dataset}
\label{tab:atyp-stmt}
\begin{tabular}{lc|c}
    \toprule
    
    Classifier & Method                  & Accuracy (\%)    \\      
    \hline
    \hline
       
    CLIP      & -                       & 0.00             \\
    LLAVA       & -                      & 0.00             \\ 
    BLIP-2     & -                       & 0.00             \\
    Flamingo   & -                       & 0.00             \\
    \hline
    FLanT5    & UH                      & 0.00             \\
    \hline
    LLama2    & UH                      & 0.00             \\
    \hline
    GPT 3.5    & UH                      & \textbf{?}     \\
    \hline
    GPT 4     & UH                      & ?            \\
\bottomrule
\end{tabular}
\end{table}
% \end{adjustwidth}

==> tables/atypic_annotation_ablation.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}


\begin{table}[!tp]%[!tp]
\centering
\scriptsize
\caption{\textbf{Impact of atypicality in VLMs on small-set.} 
%Comparing using GT atypicality stmt, predicted atpyicality stmt, wrong atpyicality stmt. 
$I$: image , $s^+$: GT atypicality, $\hat{s}$: predicted atpyicality based on $\mathcal{T}_\mathcal{V}$, $\Bar{s}$: wrong atpyicality. Accuracy on Single ARR.}\label{tab:atypicality_ablation_vlm}
\begin{tabular}{l||cccc}\toprule
 \textbf{Model }& \textbf{$I$}& \textbf{$I+s^+$}& \textbf{$I+\hat{s}$}& \textbf{$I+\Bar{s}$} \\
 \hline
 \hline
 % CLIP & 00.00 & 00.00 & 00.00 & 00.00 \\
 LLaVA & 26.00 & 35.18 & \textbf{54.28} & 28.16 \\
 InstructBLIP & 20.44 & 23.25 & \textbf{23.40} & 19.69\\
 GPT-4V & 86.87 & \textbf{89.35} & 87.24 & 86.96 \\
 \hline
 GPT-4 ($\mathcal{T}_{\mathcal{V}}$)& \textbf{96.77} & 91.42 & 96.76 & 90.20 \\

\bottomrule
\end{tabular}
\end{table}

==> tables/atypic_understanding_small_set_table.tex <==
% % %Please add the following packages if necessary:
% % % \usepackage{booktabs, multirow} % for borders and merged ranges
% % % \usepackage{soul}% for underlines
% % % \usepackage[table]{xcolor} % for cell colors
% % % \usepackage{changepage,threeparttable} % for wide tables
% % %If the table is too wide, replace \begin{table}[!htp]...\end{table} with
% % %\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
% % \begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]
% % \centering
% % \caption{Multi-label atypicality classification with llava verbalization on Small dataset}\label{tab: }
% % \scriptsize
% % \begin{tabular}{lcccccccccccccc}\toprule
% % \multirow{2}{*}{\textbf{Model}} &\multicolumn{5}{c}{\textbf{Percision}} &\multicolumn{5}{c}{\textbf{Recal}} &\multirow{2}{*}{\textbf{Percision}} &\multirow{2}{*}{\textbf{Recall}} &\multirow{2}{*}{\textbf{F1-score}}&\multirow{2}{*}{\textbf{Acc}} \\
% % \cmidrule(lrrrr){2-6}
% % \cmidrule(lrrrr){7-11   }
% % &\textbf{NA} &\textbf{TR1} &\textbf{TR2} &\textbf{OIO} &\textbf{OR} &\textbf{NA } &\textbf{TR1} &\textbf{TR2} &\textbf{OIO } &\textbf{OR} & & & \\\hline

% % \multicolumn{1}{c|}{LLava} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 h\
% % \multicolumn{1}{c|}{BLIP-2} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% % \multicolumn{1}{c|}{Flamingo} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% % \hline
% % \multicolumn{1}{c|}{LLama2} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% %  \multicolumn{1}{c|}{GPT3.5} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% % \multicolumn{1}{c|}{GPT4} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% % \bottomrule
% % \end{tabular}
% % \end{threeparttable}\end{adjustwidth}




% %Please add the following packages if necessary:
% %\usepackage{booktabs, multirow} % for borders and merged ranges
% %\usepackage{soul}% for underlines
% %\usepackage[table]{xcolor} % for cell colors
% %\usepackage{changepage,threeparttable} % for wide tables
% %If the table is too wide, replace \begin{table}[!htp]...\end{table} with

% \begin{table}[!htp]\centering
% \caption{Generated by Spread-LaTeX}\label{tab: }
% \scriptsize
% \begin{tabular}{ll|cccccccc}\toprule
% Classifier &Method &\multicolumn{2}{|c}{Precision} &\multicolumn{2}{c}{Recall} &\multicolumn{2}{c}{F1-score} &\multicolumn{2}{c}{Acc}  \\
% \cmidrule(lr){3-4}
% \cmidrule(lr){5-6}
% \cmidrule(lr){7-8}
% \cmidrule(lr){9-10}
% & &$\checkmark$ &$\times$ &$\checkmark$ &$\times$&$\checkmark$ &$\times$&$\checkmark$&$\times$ \\ 
% \midrule
% LLava &- &0.00&0.00 &0.00 &0.00 &0.00&0.00 &0.00 & 0.0\\
% BLIP-2  &- &0.00& 0.00&0.00 &0.00 &0.00& 0.00&0.00 & 0.0\\
% Flamingo  &- &0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\
% GPT4-V  &- &0.00&0.00 &0.00 & 0.00&0.00& 0.00&0.00 & 0.0\\
% \hline
% \multirow{3}{*}{Flan T5} &V,T&0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\
% &IN &0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\
% &UH &0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\

% \multirow{3}{*}{Llama 2} &V,T&0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\
% &IN &0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\
% &UH &0.00&0.00 &0.00 & 0.00&0.00&0.00 &0.00 & 0.0\\
% \hline
% \multirow{3}{*}{GPT 3.5} &V,T &41.00 &33.49 &23.71 &19.79 &29.31 &23.96 &\textbf{55.65} &\textbf{34.68}\\
% &IN &\textbf{50.16} &\textbf{47.78} &27.11 &19.29 &\textbf{30.32} &23.14 &50.40 &18.15 \\
% &UH &48.02&43.65 &28.64 &32.34 &28.45 &\textbf{28.45} &37.50 &31.05\\
% \multirow{3}{*}{GPT-4} &V,T &39.35 &34.91 &24.03 &8.86 &24.78 &13.92 &60.48 &13.71 \\
% &IN &53.55 &52.77 &26.07 &13.97 &30.17 &21.63 &59.68 &18.55\\
% &\textbf{UH} &\textbf{57.15} &\textbf{56.79} &\textbf{30.41} &30.54 &\textbf{55.42} &\textbf{56.31} &\textbf{39.77} &\textbf{} \\
% \bottomrule
% \end{tabular}
% \end{table}





% Begin table environment
\begin{table}[!htp]
    \centering
    \scriptsize
\caption{\textbf{Atypicality Understanding Tasks (MAC \& ASR) on small-set}. $\checkmark$/$\times$ denotes performance with/without No Atypicality (NA) class. Bolded numbers are the best-performing strategy per LLM.} % Table caption
    \label{tab:MAC_ASR_SMALL_SET} % Label for referencing
    % \scriptsize % Smaller font size for table content
    \begin{tabular}{lc||cccccc||c}
        \toprule
        && \multicolumn{6}{c||}{\textbf{\textit{MAC}(\%)}} & \textbf{\textit{ASR(\%)}} \\
        % Header section with merged cells for "Precision", "Recall", "F1-score", and "Acc"
        \textbf{Classifier} & \textbf{Method} & \multicolumn{2}{c}{\textbf{Precision} } & \multicolumn{2}{c}{\textbf{Recall}} & \multicolumn{2}{c||}{\textbf{F1-score }}   & \multirow{2}{*}{\textbf{Acc}} \\
        
        % Column separation lines
        % \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
        
        % Sub-header for indicating inclusion/exclusion of "No Atypicality"
        & & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ &\\ 
        
        \hline
        \hline
        % Data rows
        LLaVA \cite{liu2023visual} & - & 23.17 &28.97 & 37.58 & 46.97 & 18.90 & 23.62  & 17.00 \\
        % BLIP-2 \cite{li2023blip} & - & 33.10 & 16.38 & 40.92 & 49.69 & 15.48 & 16.59  & 32.52\\
        % MiniGPT4 \cite{zhu2024minigpt} & - & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00\\
        GPT4-V & - & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00  & 35.18\\
        \hline
        \hline
        % Multi-row entries for models with different methods
        % \multirow{3}{*}{Flan T5} & V+T & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.0 &00.00\\
        %                          & IN  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.0 &00.00\\
        %                          & UH  & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.0& 00.00\\
        % \hline
        \multirow{3}{*}{Vicuna \cite{vicuna2023}} & $V+T$ & 33.12 & 30.46 & \textbf{41.50 }& \textbf{50.60} & 21.59 & 24.70 &18.15\\
                                & $IN $  & 35.67 & \textbf{35.67} & 36.63 & 43.42 & 23.22 & 25.01  & \textbf{24.59}\\
                                 & $UH$  & \textbf{45.15} & 34.77 & 36.04 & 42.68 &\textbf{ 27.76} & \textbf{30.43}  & 20.97\\
        
        % Separation line for clarity
        \hline
        % Additional rows for more models
        \multirow{3}{*}{GPT 3.5} & $V+T$  & 41.00 & 33.49 & 23.71 & 19.79 & 29.31 & 23.96  & 51.40\\
                                 & $IN$  & \textbf{50.16} & \textbf{47.78} & 27.11 & 19.29 & \textbf{30.32} & 23.14 &51.82\\
                                 & $UH $  & 48.02 & 43.65 & \textbf{28.64} & \textbf{32.34 }&27.34 &\textbf{28.45} & \textbf{58.70}\\
        \hline
        \multirow{3}{*}{GPT-4} &$V+T$ & 39.35 & 34.91 & 24.03 & 8.86 & 24.78 & 13.92  & 50.20\\
                                &$IN$ & 53.55 & 52.77 & 26.07 & 13.97 & 30.17 & 21.63 & \textbf{51.83}\\
                                &$UH$ & \textbf{57.15} & \textbf{56.79} & \textbf{30.41}& \textbf{30.54} & \textbf{35.79} & \textbf{34.84}  & 49.37\\
\bottomrule
\end{tabular}
\end{table}
                                 

==> tables/atypical_statement_main.tex <==
% \begin{adjustwidth}{-4.5 cm}{-4.5 cm}\centering
% \begin{table}[!htb]
% \centering
% \scriptsize
% \caption{Comparative accuracies of various models in atypicality statement detection.}
% \label{tab:atyp-stmt}
% \begin{tabular}{lcc}

% \toprule
% {Model} & {Accuracy ()} \\
% \midrule
% CLIP & 54 \\
% LLAVA  & 27 \\
% Multistep Sequential LLAVA & 48.5 \\
% Sequential LLAVA & 29.9 \\
% GPT4v & 35.18 \\
% Multistep Sequential GPT4v & 64.4 \\
% GPT4 with Single Step Description & 61.2 \\
% CoT GPT4 with Single Step Description & 57.7 \\
% GPT4 with Unusual Description & 61.6 \\
% CoT GPT4 with Unusual Description  & 59.68 \\
% \bottomrule
% \end{tabular}
% \end{table}
% \end{adjustwidth}



% \begin{adjustwidth}{-4.5 cm}{-4.5 cm}
% \centering
\begin{table}[!htb]
\centering
\scriptsize
\caption{\textbf{Atypicality Statement Retrieval (ASR).} All results on the smaller dataset}
\label{tab:atyp-stmt}
\begin{tabular}{lc|c}
    \toprule
    
    Classifier & Method                  & Accuracy (\%)    \\      
    \hline
    \hline
       
    % CLIP      & -                       & 54.00             \\
    LLaVA       & -                      & 17.00             \\ 
    BLIP-2     & -                       & 32.52             \\
    MiniGPT4   & -                       & 0.00             \\
    GPT4-V     & -                       & 35.18             \\
    \hline
    FLanT5    
               & V+T     & 0.00             \\
               & IN                      & 0.00             \\
               & UH                      & 0.00             \\
    \hline
    Vicuna     
               & V+T    & 0.00             \\
               & IN                      & 0.00             \\
               & UH                      & 0.00             \\
    \hline
    GPT 3.5    
               & V+T     & 51.41     \\
               & IN                      & 51.82     \\
               & UH                      & \textbf{58.70}     \\
    \hline
    GPT 4     
               & V+T     & 50.20            \\
               & IN                      & \textbf{51.83 }           \\
               & UH                      & 49.37            \\
\bottomrule
\end{tabular}
\end{table}
% \end{adjustwidth}

==> tables/more_vlms.tex <==
% \setlength{\tabcolsep}{1pt}
\begin{table}
\centering

%is based on $UH$. LLaVA + GPT-4 verbalization. 
%, $\hat{s}_{UH}$: atypc prediction based on UH}
\vspace{-0.25cm}
\scriptsize
\begin{tabular}{lc||c|c|c}
\toprule
 \textbf{classifier} & \textbf{Verb}. & \multicolumn{3}{c}{\textit{\textbf{Precision@k}}} \\

&&\textbf{k=1} & \textbf{k=2} &\textbf{k=3}\\
\hline
\hline
 \multirow{1}{*}{InternVL-Chat-V1-1} 
 &$I$  & 52.22 & 32.79 & 22.17 \\
 % \multirow{1}{*}{InternVL2‑8B} &$I$  & 92.12 & 76.66 & 56.19\\
 % \hline
\multirow{2}{*}{Vicuna} 
&$\mathcal{T}_\mathcal{V}$ (Ours) & 67.38  & 44.01 & 29.94 \\

& $\mathcal{T}_\mathcal{V} + \hat{s}_{IN}$ (Ours) & \textbf{68.32 }& \textbf{44.52} &  \textbf{30.25} 

\\

% \multirow{1}{*}{InternLM} 
% &$\mathcal{T}_\mathcal{V}$ (Ours) & \textbf{93.60}  & \textbf{78.20} & \textbf{57.20} \\

% \multirow{1}{*}{LLAMA3}&$\mathcal{T}_\mathcal{V}$ (Ours) & 85.44 & 65.49 & 46.03\\
\hline
\multirow{2}{*}{GPT-4} 
  &$\mathcal{T}_\mathcal{V}$ (Ours) & 93.99& 86.35 & 72.96 \\
  & $\mathcal{T}_\mathcal{V} +\hat{s}_{IN}$ (Ours) & \textbf{95.54} & \textbf{87.55} & \textbf{74.62} \\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Additional VLMs for ARR on Full-set}}
\label{tab:rebuttal_more_vlms}
\end{table}

==> tables/more_vlms_small_set.tex <==
% \setlength{\tabcolsep}{1pt}
\begin{table}
\centering

%is based on $UH$. LLaVA + GPT-4 verbalization. 
%, $\hat{s}_{UH}$: atypc prediction based on UH}
\vspace{-0.25cm}
\scriptsize
\begin{tabular}{lc||c|c|c}
\toprule
 \textbf{classifier} & \textbf{Verb}. & \multicolumn{3}{c}{\textit{\textbf{Precision@k}}} \\

&&\textbf{k=1} & \textbf{k=2} &\textbf{k=3}\\
\hline
\hline
 \multirow{1}{*}{LLaVA 1.6} 
 &$I$  & 74.79 & 52.00 &35.73 \\
 % \multirow{1}{*}{InternVL2‑8B} &$I$  & 92.12 & 76.66 & 56.19\\
 % \hline
\multirow{1}{*}{Vicuna} 
&$\mathcal{T}_\mathcal{V}$ (Ours) & \textbf{86.40} & \textbf{62.40} & \textbf{43.19} \\
\hline
% \multirow{1}{*}{InternLM} 
% &$\mathcal{T}_\mathcal{V}$ (Ours) & \textbf{93.60}  & \textbf{78.20} & \textbf{57.20} \\

\multirow{1}{*}{InternVL2-8B}
&$I$ & 91.12 & 75.40 & 55.64\\
\multirow{1}{*}{InternLM}
&$\mathcal{T}_\mathcal{V}$ (Ours) & \textbf{93.60} & \textbf{78.20} & \textbf{57.20}\\
\bottomrule
\end{tabular}
\vspace{-0.2cm}
\caption{\textbf{Additional VLMs for ARR on Small-set}. InternLM is `InternLM2-5-7b-chat'.}
\label{tab:rebuttal_more_vlms_smallset}
\vspace{-4pt}
\end{table}

==> tables/multi_label_classificaiton_main.tex <==
%Please add the following packages if necessary:
% \usepackage{booktabs, multirow} % for borders and merged ranges
% \usepackage{soul}% for underlines
% \usepackage[table]{xcolor} % for cell colors
% \usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}


% \begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]
% \centering
% \caption{Multi-label atypicality classification with llava verbalization on Large dataset}\label{tab: }
% \scriptsize
% \begin{tabular}{lcccccccccccccc}\toprule
% \multirow{2}{*}{\textbf{Model}} &\multicolumn{5}{c}{\textbf{Percision}} &\multicolumn{5}{c}{\textbf{Recal}} &\multirow{2}{*}{\textbf{Percision}} &\multirow{2}{*}{\textbf{Recall}} &\multirow{2}{*}{\textbf{F1-score}}&\multirow{2}{*}{\textbf{Acc}} \\
% \cmidrule(lrrrr){2-6}
% \cmidrule(lrrrr){7-11}
% &\textbf{NA} &\textbf{TR1} &\textbf{TR2} &\textbf{OIO} &\textbf{OR} &\textbf{NA } &\textbf{TR1} &\textbf{TR2} &\textbf{OIO } &\textbf{OR} & & & \\\hline

% \multicolumn{1}{c|}{LLava} &0.00 &33.49 &23.72 &18.66 &40.00 &0.00 &20.29 &69.57 &96.71 &1.32 &23.17 &37.58 &18.90 & 37.93 \\
% \multicolumn{1}{c|}{BLIP-2} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% \multicolumn{1}{c|}{Flamingo} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% \hline
% \multicolumn{1}{c|}{LLama2} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
%  \multicolumn{1}{c|}{GPT3.5} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% \multicolumn{1}{c|}{GPT4} &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 &0.00 \\
% \bottomrule
% \end{tabular}
% \end{threeparttable}\end{adjustwidth}

==> tables/rebuttal_llava.tex <==

% \begin{table}
% \centering
% \caption{\textbf{LLaVA classifier with different verbalization approaches on action-reason retrieval task}.  
% }

% \label{tab:llava_multi_selection_action_reason}

% %is based on $UH$. LLaVA + GPT-4 verbalization. 
% %, $\hat{s}_{UH}$: atypc prediction based on UH}
% \scriptsize
% \begin{tabular}{lc||ccc||ccc}
% \toprule
%  \textbf{classifier} & \textbf{Verb}. & \multicolumn{3}{c||}{\textit{\textbf{Precision@k}}} & \multicolumn{3}{c}{\textit{\textbf{Top-k Acc}}} \\

% &\textbf{k=1}&\textbf{k=2} &\textbf{k=3} &\textbf{k=1}&\textbf{k=2} &\textbf{k=3}\\
% \hline
% \hline
%  \multirow{4}{*}{LLaVA \cite{liu2023improvedllava}}& $I$& 58.50 & 37.24 & 24.97   & 26.90  & 47.67     & 58.50\\
%  & $I+V+T$&55.95 &36.09 &24.26 & 26.77 & 45.42 & 55.95\\
%  & $I+IN$ &\textbf{58.80} & 37.33 & 25.32 & 26.60 &45.96 & \textbf{58.80}\\
%  & $I+IN+UH+V+T$ &57.52 & \textbf{38.44} & \textbf{25.87} & \textbf{27.52} &\textbf{48.16} & 57.52\\
%  \hline
%  \multirow{4}{*}{Vicuna \cite{vicuna2023}}& $I$& 58.50 & 37.24 & 24.97   & 26.90  & 47.67     & 58.50\\
%  & $I+V+T$&55.95 &36.09 &24.26 & 26.77 & 45.42 & 55.95\\
%  & $I+IN$ &\textbf{58.80} & 37.33 & 25.32 & 26.60 &45.96 & \textbf{58.80}\\
%  & $I+IN+UH+V+T$ &57.52 & \textbf{38.44} & \textbf{25.87} & \textbf{27.52} &\textbf{48.16} & 57.52\\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}
% \centering
% \caption{{Action-reason Retrieval on full-set}.  
% }

% \label{tab:llava_multi_selection_action_reason}

% %is based on $UH$. LLaVA + GPT-4 verbalization. 
% %, $\hat{s}_{UH}$: atypc prediction based on UH}
% \scriptsize
% \begin{tabular}{lc||cc||cc}
% \toprule
%  \textbf{classifier} & \textbf{Verb}. & \multicolumn{2}{c||}{\textit{\textbf{Precision@k}}} & \multicolumn{2}{c}{\textit{\textbf{Top-k Acc}}} \\

% &&\textbf{k=2} &\textbf{k=3} &\textbf{k=1}&\textbf{k=2}\\
% \hline
% \hline
%  \multirow{4}{*}{LLaVA \cite{liu2023improvedllava}}& $I$&  37.24 & 24.97   & 26.90  & 47.67\\
%  & $I+V+T$&36.09 &24.26 & 26.77 & 45.42\\
%  & $I+IN$& 37.33 & 25.32 & 26.60 &45.96\\
%  & $I+IN+UH+V+T$ & \textbf{38.44} & \textbf{25.87} & \textbf{27.52} &\textbf{48.16} \\
%  \hline
% \multirow{2}{*}{Vicuna~\cite{vicuna2023}}&$V + T$& 40.71 &27.57 & 21.49 & 43.41\\
%    &$\mathcal{T}_\mathcal{V}$ (Ours) &44.01 & 29.94  & 23.20 & 41.95\\
% \hline
% \multirow{2}{*}{GPT-4} &$V+T$&84.42 &70.50  & 71.50 & 89.87\\
%  &$\mathcal{T}_\mathcal{V}$ (Ours) &86.35 &72.96 & 74.94 & 91.16 \\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}
% \centering
% \caption{{Action-reason Retrieval on full-set}.  
% }

% \label{tab:llava_multi_selection_action_reason}

% %is based on $UH$. LLaVA + GPT-4 verbalization. 
% %, $\hat{s}_{UH}$: atypc prediction based on UH}
% \scriptsize
% \begin{tabular}{lc||cc||cc}
% \toprule
%  \textbf{classifier} & \textbf{Verb}. & \multicolumn{2}{c||}{\textit{\textbf{Precision@k}}} & \multicolumn{2}{c}{\textit{\textbf{Top-k Acc}}} \\

% &&\textbf{k=2} &\textbf{k=3} &\textbf{k=1}&\textbf{k=2}\\
% \hline
% \hline
%  \multirow{2}{*}{LLaVA \cite{liu2023improvedllava}}& $I$&  37.24 & 24.97   & 26.90  & 47.67\\
% &$\mathcal{T}_\mathcal{V}$ (Ours) &37.37 &25.14 & 27.49 & 47.07 \\
%  \hline
% \multirow{1}{*}{Vicuna~\cite{vicuna2023}}&$\mathcal{T}_\mathcal{V}$ (Ours) &44.01 & 29.94  & 23.20 & 41.95\\
% \hline
% \multirow{2}{*}{GPT-4}&$\mathcal{T}_\mathcal{V}$ (Ours) &\textbf{86.35} &\textbf{72.96} & \textbf{74.94} & \textbf{91.16} \\
% \bottomrule
% \end{tabular}
% \end{table}




% \begin{table}[!tp]
% \vspace{-0.25cm}
% \centering
% \caption{{ARR, MAC, and ASR tasks on full-set}.  
% }

% \label{tab:llava_multi_selection_action_reason}

% %is based on $UH$. LLaVA + GPT-4 verbalization. 
% %, $\hat{s}_{UH}$: atypc prediction based on UH}
% \scriptsize
% \begin{tabular}{lc||cc||c||c}
% \toprule
%  \textbf{classifier} & \textbf{Verb}. & \multicolumn{2}{c||}{\textit{\textbf{ARR}}} &  \textit{\textbf{MAC}} & \textbf{ASR}\\

% &&\textbf{prec@2} &\textbf{prec@3} &\textbf{F1-score}&\textbf{Acc.}\\
% \hline
% \hline
%  \multirow{4}{*}{LLaVA }& $I$ & 37.24 & 24.97   & 21.24  & 18.83\\
% & $I + IN$ & \_ & \_ & \textbf{27.05} & \textbf{20.90} \\
% & $I + UH$ &  \_ & \_   & 24.16  & 17.90\\
% & $ I + \mathcal{T}_\mathcal{V}$ &  \textbf{37.37} & \textbf{25.14}  & \_ & \_\\
%  \hline
% \multirow{3}{*}{Vicuna} & $IN$  & \_ & \_  & 34.51 & 23.29\\
% & $UH$ & \_ & \_  & 27.35 & 14.47\\
% & $ \mathcal{T}_\mathcal{V}$ &  44.01 & 29.94 & \_  & \_\\
% \hline
% \multirow{3}{*}{GPT-4}&$IN$  & \_ & \_ & 30.58 & \textbf{57.70}\\
% &$UH$ & \_ & \_  & \textbf{34.62} & 56.89\\
% & $\mathcal{T}_\mathcal{V}$  &\textbf{86.35} &\textbf{72.96}  & \_ & \_ \\

% \bottomrule
% \end{tabular}
% \vspace{-0.5cm}
% \end{table}


% \begin{table}[!tp]
% \centering
% % \caption{ARR, MAC, and ASR tasks on full-set.}
% \label{tab:llava_multi_selection_action_reason}
% \begin{minipage}[b]{0.4\textwidth}
%     \centering
%     \caption{MAC and ASR Tasks}
%     \scriptsize
%     \begin{tabular}{lc||c||c}
%     \toprule
%      \textbf{CLS.} & \textbf{Verb}. & \textbf{F1-score} & \textbf{Acc.}\\
%     \hline
%     \multirow{2}{*}{LLaVA } & $I + IN$ & \textbf{27.05} & \textbf{20.90} \\
%                             & $I + UH$ & 24.16 & 17.90\\
%     \hline
%     \multirow{2}{*}{Vicuna} & $IN$ & 34.51 & 23.29\\
%                             & $UH$ & 27.35 & 14.47\\
%     \hline
%     \multirow{2}{*}{GPT-4} & $IN$ & 30.58 & \textbf{57.70}\\
%                            & $UH$ & \textbf{34.62} & 56.89\\
%     \bottomrule
%     \end{tabular}
% \end{minipage}
% \begin{minipage}[b]{0.4\textwidth}
%     \centering
%     \caption{ARR Task}
%     \scriptsize
%     \begin{tabular}{lc||cc}
%     \toprule
%      \textbf{CLS.} & \textbf{Verb}. & \textbf{p@2} & \textbf{p@3}\\
%     \hline
%      \multirow{1}{*}{LLaVA} & $I + \mathcal{T}_\mathcal{V}$ & \textbf{37.37} & \textbf{25.14} \\
%     \hline
%     \multirow{1}{*}{Vicuna} & $\mathcal{T}_\mathcal{V}$ & 44.01 & 29.94 \\
%     \hline
%     \multirow{1}{*}{GPT-4} & $\mathcal{T}_\mathcal{V}$  & \textbf{86.35} & \textbf{72.96} \\
%     \bottomrule
%     \end{tabular}
% \end{minipage}
% \end{table}

\begin{table}[!tp]
\vspace{-0.35cm}
\centering
% \caption{ARR, MAC, and ASR tasks on full-set.}
\label{tab:llava_multi_selection_action_reason}

\begin{minipage}[b]{0.50\linewidth}
    \centering
    \caption{MAC (F1), ASR (Acc)}
    \label{tab:atyp_tasks}
    \scriptsize
    \begin{tabular}{lc||c||c}
    \toprule
     \textbf{CLS.} & \textbf{Verb}. & \textbf{MAC} & \textbf{ASR}\\
    \midrule
    \multirow{2}{*}{LLaVA } & $I + IN$ & 27.05 & 20.90 \\
                            & $I + UH$ & 24.16 & 17.90\\
    \midrule
    \multirow{2}{*}{Vicuna} & $IN$ & 34.51 & 23.29\\
                            & $UH$ & 27.35 & 14.47\\
    \midrule
    \multirow{2}{*}{GPT-4} & $IN$ & 30.58 & \textbf{57.70}\\
                           & $UH$ & \textbf{34.62} & 56.89\\
    \bottomrule
    \end{tabular}
\end{minipage}%
\hspace{0.66cm}
\begin{minipage}[b]{0.4\linewidth}
    \centering
    
    \caption{ARR }
    \label{tab:ARR_task}
    \scriptsize
    \begin{tabular}{lc||c}
    \toprule
     \textbf{CLS.} & \textbf{Verb}. & \textbf{p@3}\\
    \midrule
     LLaVA & $I + \mathcal{T}_\mathcal{V}$ & 25.14 \\
    \midrule
    Vicuna & $\mathcal{T}_\mathcal{V}$  & 29.94 \\
    \midrule
    GPT-4 & $\mathcal{T}_\mathcal{V}$  &  \textbf{72.96} \\
    \bottomrule
    \end{tabular}
\end{minipage}
\end{table}

%  Complete

% \begin{table}[!htp]\centering
% \caption{\textbf{ARR on full-set. Predicted atypicality statement $\hat{s}$ is based on $UH$. LLaVA + GPT-4 verbalization} Results on the full-set. BLIP-2's result is generated with Single prediction prompt (i.e. just predict one a+r stmt, as multi one fails)}\label{tab: full_multi_selection_action_reason}
% \scriptsize
% \begin{tabular}{lc||ccc||ccc}
% \toprule
% \textbf{Classifier} &\textbf{Verb}. & \multicolumn{3}{c||}{\textit{\textbf{Precision@k}}} & \multicolumn{3}{c}{\textit{\textbf{Top-k Acc}}} \\

% & &\textbf{k=1}&\textbf{k=2} &\textbf{k=3} &\textbf{k=1}&\textbf{k=2} &\textbf{k=3}\\
% \hline
% \hline
%  \multirow{2}{*}{CLIP \cite{radford2021learning}}  &$I$ & 61.04 & 33.86 & 22.66 & 23.72 & 44.61 & 61.04\\
%  &$I+\hat{s}_{UH}$ & 42.47 & 22.47 &14.98 & 13.44 & 28.51 & 42.47\\
%  \multirow{2}{*}{CLIP (KAFA)}& $I+T$&46.15 &24.36 &16.24 & 15.15 & 31.25 & 46.15\\
%  &$I+T+\hat{s}_{UH}$ &\textbf{56.51} &\textbf{30.39} &\textbf{20.26}& 19.35 & 39.81 & 56.51 \\\hline
 
% \multirow{2}{*}{LLaVA \cite{liu2023visual}} &$I$ &37.24 &37.24 &24.97& 26.90 & 47.67 & 37.24 \\
%      &$I +\hat{s}_{UH}$ &60.72 &38.29 &25.78& 28.34 & 47.03 & 36.22 \\
% \multirow{2}{*}{BLIP-2\cite{li2023blip}} &$I$ &0.00 & Failed & Failed & Failed & Failed & Failed \\
%  &$I +\hat{s}_{UH}$ & 0.00 &Failed &Failed & Failed & Failed & Failed \\
% \multirow{2}{*}{MiniGPT4~\cite{zhu2024minigpt}} &$I$& 0.00 & 0.00 & 0.00 & 00.00 & 00.00 & 00.00\\
%  &$I +\hat{s}_{UH}$ & 0.00 & 0.00 & 0.00 & 00.00 & 00.00 & 00.00 \\
%  \hline

% \multirow{3}{*}{Vicuna}&$V + T$& 64.13 & 40.71 &27.57 & 21.49 & 43.41 & 64.13\\
%  &$\mathcal{T}_\mathcal{V}$ & 68.49 & 44.52 & 30.37  & 24.06 & 43.24 & 68.49 \\
%  &$\mathcal{T}_\mathcal{V}+\hat{s}_{UH}$& \textbf{69.09} & \textbf{45.16} & \textbf{30.71} & 24.49 & 43.84 & 69.09 
%  \\\hline
% \multirow{3}{*}{GPT 3.5} &$V + T $& 0.00 & 0.00 & 0.00 & 00.00 & 00.00 & 00.00\\
%  &$\mathcal{T}_\mathcal{V}$ & 0.00 & 0.00 & 0.00 & 00.00 & 00.00 & 00.00\\
%  &$\mathcal{T}_\mathcal{V} + \hat{s}_{UH}$ & 0.00 & 0.00 & 0.00 & 00.00 & 00.00 & 00.00\\
%  \hline
% \multirow{3}{*}{GPT 4} &$V+T$&93.73 &84.42 &70.50  & 71.50 & 89.87 & 93.73\\
%  &$\mathcal{T}_\mathcal{V}$ &93.99 &\textbf{86.35} &\textbf{72.96} & \textbf{74.94} & 91.16 & 93.99 \\
%  &$\mathcal{T}_\mathcal{V} + \hat{s}_{UH}$&\textbf{94.42} &85.95 &72.31  & 74.31 & \textbf{91.84} & \textbf{94.42}\\
% \bottomrule
% \end{tabular}
% \end{table}




    






==> tables/supp_tab_gpt4v_complete.tex <==
\setlength{\tabcolsep}{1pt}
\begin{table}[!htp]\centering
\caption{GPT4-V experiments}\label{tab:supp_gpt4v_results}
\scriptsize
\begin{tabular}{lc||ccc||c||ccc|ccc||c}\toprule
\multirow{3}{*}{\textbf{Classifier}}& \multirow{3}{*}{\textbf{Method}}& \multicolumn{3}{c||}{\textbf{\textit{MAC}}}& \textbf{\textit{ASR}} &\multicolumn{6}{c||}{\textbf{\textit{ARR multi}}}  & \textbf{\textit{ARR Single}}\\

& & \multirow{2}{*}{\textbf{precision}} & \multirow{2}{*}{\textbf{recall}} & \multirow{2}{*}{\textbf{f1-score}} &Acc& \multicolumn{3}{c}{\textbf{precision@k}} & \multicolumn{3}{c||}{\textbf{Top-k acc}}&\multirow{2}{*}{\textbf{Acc}} \\
 & & & & & &\textbf{k=1} &\textbf{k=2 }&\textbf{k=3} &\textbf{k=1} &\textbf{k=2} &\textbf{k=3} \\
\hline
\hline
LLaVA &- &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 \\
GPT4-V &- &0 &0 &0 &0 &0 &0 &0 &0 &0 &0&0 \\
GPT-4 &$\mathcal{T}_\mathcal{V}$ &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0\\
GPT-4 & $\mathcal{T}_\mathcal{V} + \hat{s}_{IN}$ &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 &0 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/tab_combined_gpt4v_atypic_ablation.tex <==

% \begin{table}[!htp]
% \centering
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \caption{\textbf{GPT-4V verbalization in ARR on small set}. We prompt GPT-4V to generate \textit{V}, \textit{T}, \textit{UH}, and \textit{IN}. Then we generate the final verbalization as explained in Sec.~\ref{sec:proposed-approach} using GPT-4 model.}\label{tab:action_reason_gpt4v}
%     \scriptsize
%     \begin{tabular}{l||ccc|ccc}\toprule
%     \multirow{3}{*}{\textbf{Classifier}}  & \multicolumn{6}{c}{\textbf{\textit{Multi}}}\\ % & \textbf{\textit{Single}} \\
%     &  \multicolumn{3}{c}{\textbf{\textit{precision@k}}} & \multicolumn{3}{c}{\textbf{\textit{Top-k acc}}} \\ % & \multirow{2}{*}{\textbf{Acc}} \\
%     &  \textbf{k=1} & \textbf{k=2} & \textbf{k=3} & \textbf{k=1} & \textbf{k=2} & \textbf{k=3} \\ %& \\
%     \hline
%     \hline
%     LLaVA  & 59.67 & 38.27 & 26.06 & 32.92 & 48.14 & 59.67 \\ %& 26.00 \\
%     GPT-4V & 56.40 & 38.00 & 26.80 & 22.00 & 49.60 & 56.40 \\ %& 90.00 \\
%     GPT-4  $\mathcal{T}_\mathcal{V}$  & 97.58 & 90.72 & 76.61 & 81.04 & 92.74 & 97.58  \\ %& 97.90 \\
%     % GPT-4 $\mathcal{T}_\mathcal{V} + \hat{s}_{UH}$ & 0 & 0 & 0 & 0 & 0 & 0 \\ % & 0 \\
%     \bottomrule
%     \end{tabular}
% \end{minipage}\hfill
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \caption{\textbf{Impact of atypicality in VLMs on small-set.} Comparing using GT atypicality stmt, predicted atpyicality stmt, wrong atpyicality stmt. $I$: image, $s^+$: GT atypicality, $\hat{s}$: predicted atypicality, $\Bar{s}$: wrong atypicality. Accuracy on Single ARR.}\label{tab:atypicality_ablation_vlm}
%     \scriptsize
%     \begin{tabular}{l||cccc}\toprule
%     \textbf{Model} & \textbf{$I$} & \textbf{$I+s^+$} & \textbf{$I+\hat{s}$} & \textbf{$I+\Bar{s}$} \\
%     \hline
%     \hline
%     % CLIP & 00.00 & 00.00 & 00.00 & 00.00 \\
%     LLaVA & 26.00 & 35.18 & \textbf{54.28} & 28.16 \\
%     InstructBLIP & 20.44 & 23.25 & \textbf{23.40} & 00.00 \\
%     GPT-4V & 86.87 & 89.35 & 87.24 & 86.96 \\
%     \hline
%     GPT-4 ($\mathcal{T}_{\mathcal{V}}$) & 93.88 & 0.00 & 96.36 & 90.69 \\
%     \bottomrule
%     \end{tabular}
% \end{minipage}
% \end{table}


